High-probability Bounds for Non-Convex Stochastic Optimization with Heavy Tails

We consider non-convex stochastic optimization using first-order algorithms for which the gradient estimates may have heavy tails. We show that a combination of gradient clipping, momentum, and normalized gradient descent yields convergence to critical points in high-probability with best-known rates for smooth losses when the gradients only have bounded $\mathfrak{p}$th moments for some $\mathfrak{p}\in(1,2]$. We then consider the case of second-order smooth losses, which to our knowledge have not been studied in this setting, and again obtain high-probability bounds for any $\mathfrak{p}$. Moreover, our results hold for arbitrary smooth norms, in contrast to the typical SGD analysis which requires a Hilbert space norm. Further, we show that after a suitable "burn-in" period, the objective value will monotonically decrease for every iteration until a critical point is identified, which provides intuition behind the popular practice of learning rate "warm-up" and also yields a last-iterate guarantee.

==> old_sgd.tex <==
\section{Normalized SGD}

First, we present our actual algorithm. The rest of this manuscript is devoted to its analysis.

\begin{algorithm}
   \caption{Normalized SGD with Clipping}
   \label{alg:normalized}
   \begin{algorithmic}
      \STATE{\bfseries Input: } Initial Point $\bw_1$, learning rate $\eta$, momentum parameter $\beta$, clipping threshold $\tau$, outlier thresholds $\gamma$, $k$. I think it is safe to set $\gamma = \tau$, $k$ some constant like 2 or so. $\tau$ should perhaps be $O(\sigma/(1-\beta)^{1/\power})$, where we believe $\power$th moment of gradient is at most $\sigma^\power$: $\tau$ is \emph{not small} - clipping should not happen too often (maybe target about 3/4 of iterations are not clipped).
      \STATE Set $\bm_1 = \nabla f(\bx_1, \xi_1)$.
      \STATE Set $\bw_2 = \bw_1 - \eta \frac{\bm_1}{\|\bm_1\|}$.
      \STATE Set $C=0$
      \FOR{$t=2\dots T$}
      \STATE Set $\bg_t = \nabla f(\bw_t ,\xi_t)$.
      \STATE Set $s_t=\one[\|\bg_t-\bm_t\|\le \gamma]$.
      \STATE $C\gets C+1$.
      \IF{$\frac{1}{C}\sum_{t'=t-C+1}^t s_{t'} < \frac{k}{\sqrt{C}}+\beta^C + \frac{1}{4}$}
      \STATE \text{// concentration bound check to make sure that the initial gradient estimate is ok.}
      \STATE \text{//This check should only fail (i.e., execute this code block) a small number of times at the start of the run.}
      \STATE \text{//May want to consider some kind of ``hard reset'' where we actually go back to the first iterate upon upon failure.}
      \STATE Set $\bm_t = \bg_t$.
      \STATE Set $C=0$.
      \ELSE
      \STATE Set $\bg^{\text{ clip}}_t=\bm_{t-1} + \frac{\bg_t-\bm_{t-1}}{\|\bg_t-\bm_{t-1}\|}\min\left(\tau, \|\bg_t -\bm_{t-1}\|\right)$
      \STATE Set $\bm_t = \beta \bm_{t-1} + (1-\beta) \bg^{\text{ clip}}_t$.
      \ENDIF
      \STATE Set $\bw_{t+1} = \bw_t - \eta \frac{\bm_t}{\|\bm_t\|}$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}


Now we sketch the analysis, ignoring all constants and log factors:
\begin{Theorem}\label{thm:sgd}
Suppose $\bg_t$ is such that $\E[\|\bg_t - \nabla F(\bw_t)\|^\power]\le \sigma^\power$ for all $t$ for some $\alpha \in (1,2]$ for some $\sigma>0$. Then with $\beta = 1-\alpha$ for $\alpha = \frac{M}{T^{\frac{\power}{3\power-2}}}$ for sufficiently small $M$, $\eta = \frac{\sqrt{\alpha}}{\sqrt{T}}$ ($M$ sufficiently small that $\eta \le \frac{\sigma}{L}$), and $\tau = \frac{\sigma}{\alpha^{1/\power}}$, then with probability at least $1-\delta$,
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|\le O\left(\frac{1}{T^{\frac{\power-1}{3\power-2}}}\right)
\end{align*}
\end{Theorem}

\begin{proof}
Define $\hat \epsilon_t = \bm_t - \nabla F(\bw_t)$ and define $\epsilon_t = \bg^{\text{ clip}}_t-\nabla F(\bw_t)$.
% Notice that by our assumptions, we have
% \begin{align*}
%     \E[\|\epsilon_t\|^\power]&\le \sigma^\power\\
%     \E[\langle \epsilon_i,\epsilon_j\rangle]&=0\ \text{ for }i\ne j
% \end{align*}
Further, define $S(a,b) = \nabla F(a)-\nabla F(b)$. By smoothness, we must have $\|S(\bw_t,\bw_{t+1})\|\le L\|\bw_t-\bw_{t+1}\|=\eta L$ for all $t$.
With this notation, we have the following recursive formulation for any $t\ge 1$:
\begin{align*}
    \bm_{t+1} &= (1-\alpha) (\nabla F(\bw_t) + \hat \epsilon_t) + \alpha\bg^{\text{ clip}}_{t+1}\\
    &=\nabla F(\bw_{t+1}) + (1-\alpha)(S(\bw_t,\bw_{t+1})+\hat \epsilon_t) + \alpha\epsilon_{t+1}\\
    \hat \epsilon_{t+1}&= (1-\alpha)S(\bw_t,\bw_{t+1})+(1-\alpha)\hat \epsilon_t + \alpha \epsilon_{t+1}
\end{align*}
Now, we unravel the recursion for $t$ iterations:
\begin{align*}
    \hat \epsilon_{t+1}&=(1-\alpha)^t\hat \epsilon_1 +\alpha\sum_{t'=0}^{t-1} (1-\alpha)^{t'} \epsilon_{t+1-t'}+ (1-\alpha)\sum_{t'=0}^{t-1}(1-\alpha)^{t'} S(\bw_{t-t'},\bw_{t+1-t'})
\end{align*}
Next, take the magnitude of both sides and use triangle inequality:
\begin{align*}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t\|\epsilon_1\| +\alpha\left\|\sum_{t'=0}^{t-1} (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|+ (1-\alpha)\eta L \sum_{t'=0}^{t-1}(1-\alpha)^{t'}
\end{align*}
Where in the above we have observed that $\hat\epsilon_1=\epsilon_1$. 

Suppose that at some point when we reset, $\|\bg_t-\nabla F(\bw_t)\| \le K\sigma $ for some $K$. Note that this fails to happen with probability at most $\sigma^\power/K^\power$ at every reset. Then we claim that with high probability we will never reset again, and that $\|\hat \epsilon_t\|\le somthing nice$ for all $t$. Re-index so that this putative last reset is $t=1$. Then by induction on $T$:

By Markov inequality and Lemma \ref{thm:threshold}, ignoring constants and applying union bound appropriately, we have with probability at least $1-\delta$:
\begin{align*}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t \|\epsilon_1\| + \alpha \left(\tau + \sigma^{\power/2}\sqrt{\sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}\tau^{2-\power}} + \sqrt{\sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}\|\bm_{t-t'} - \nabla F(\bw_{t-t'})\|^\power \tau^{2-\power}}\right.\\
    &\quad\quad+ \left.\frac{\sum_{t'=0}^{t-1}(1-\alpha)^{\power t'} (\sigma^\power + \|\bm_{t-t'} - \nabla F(\bw_{t-t'})\|^\power)}{\tau^{\power -1}}\right)
    \intertext{Observe that $\|\bm_{t-t'} - \nabla F(\bw_{t-t'})\|\le \|\hat \epsilon_{t-t'}\| + \eta L$:}
    &\le (1-\alpha)^t \|\epsilon_1\| + \alpha \left(\tau + \sigma^{\power/2}\sqrt{\sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}\tau^{2-\power}} + \sqrt{2\sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}(\|\hat \epsilon_{t-t'}\|^\power + L^\power \eta^\power) \tau^{2-\power}}\right.\\
    &\quad\quad\left.+ \frac{\sum_{t'=0}^{t-1}(1-\alpha)^{\power t'} (\sigma^\power + 2(\|\hat \epsilon_{t-t'}\|^\power + L^\power \eta^\power))}{\tau^{\power -1}}\right)\\
    &\le (1-\alpha)^t \|\epsilon_1\| + \alpha \tau + \sqrt{\alpha\tau^{2-\power}}\sigma^{\power/2}+ \alpha \sqrt{2\sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}(\|\hat \epsilon_{t-t'}\|^\power + L^\power \eta^\power) \tau^{2-\power}}\\
    &\quad\quad+ \frac{ \sigma^\power + 2L^\power\eta^\power+ \sum_{t'=0}^{t-1}2\alpha (1-\alpha)^{\power t'}\|\hat \epsilon_{t-t'}\|^\power}{\tau^{\power -1}}\\
    &\le (1-\alpha)^t \|\epsilon_1\| + \alpha \tau + \sqrt{\alpha\tau^{2-\power}}\sigma^{\power/2}+ \sqrt{\alpha 2 L^\power \eta^\power \tau^{2-\power}}+\alpha\sqrt{2\sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}\|\hat \epsilon_{t-t'}\|^\power\tau^{2-\power}}\\
    &\quad\quad+ \frac{ \sigma^\power + 2L^\power \eta^\power + \sum_{t'=0}^{t-1}2\alpha(1-\alpha)^{\power t'} \|\hat \epsilon_{t-t'}\|^\power}{\tau^{\power -1}}
    \intertext{Use the value $\tau = \frac{\sigma}{\alpha^{1/\power}}$:}
    &\le (1-\alpha)^t \|\epsilon_1\| + (3\sigma +2L^\power \eta^\power \sigma^{1-\power}+\sqrt{2\sigma^{2-\power}L^\power \eta^\power})\alpha^{1-1/\power} +\alpha^{\frac{3}{2}-1/\power}\sqrt{2\sigma^{2-\power}\sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}\|\hat \epsilon_{t-t'}\|^\power}\\
    &\quad\quad+ \sum_{t'=0}^{t-1}2\alpha^{2-1/\power}\sigma^{1-\power}(1-\alpha)^{\power t'} \|\hat \epsilon_{t-t'}\|^\power
    \intertext{using $\eta \le  \frac{\sigma}{L}$:}
    &\le (1-\alpha)^t \|\epsilon_1\| +7\sigma\alpha^{1-1/\power} +\alpha^{\frac{3}{2}-1/\power}\sqrt{2\sigma^{2-\power}\sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}\|\hat \epsilon_{t-t'}\|^\power}+ \sum_{t'=0}^{t-1}2\alpha^{2-1/\power}\sigma^{1-\power}(1-\alpha)^{\power t'} \|\hat \epsilon_{t-t'}\|^\power    
\end{align*}
Let us suppose for purposes of induction that for all $\tind\le t$:
\begin{align*}
    \|\hat \epsilon_\tind\|\le (1-\alpha)^{\tind -1}\|\epsilon_1\| + C\alpha^{1-1/\power}
\end{align*}
Clearly, the statement is true for $t=1$. Now, we have for any $t'\le t$:
\begin{align*}
    \|\hat \epsilon_{t-t'}\|^\power &\le 2(1-\alpha)^{(t-t'-1)\power}\|\epsilon_1\|^\power + 2 C^\power\alpha^{\power - 1}\\
    \sum_{t'=0}^{t-1} (1-\alpha)^{\power t'}\|\hat \epsilon_{t-t'}\|&\le2 C^\power \alpha^{\power-2}+ \sum_{t'=0}^{t-1}2(1-\alpha)^{(t-1)\power}\|\epsilon_1\|^\power \\
    &\le2 C^\power \alpha^{\power-2}+ 2\frac{\|\epsilon_1\|^\power}{\alpha}
\end{align*}
Plugging this in, we have:
\begin{align*}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t \|\epsilon_1\| +7\sigma\alpha^{1-1/\power} +2\alpha^{\frac{1+p}{2}-1/\power}\sqrt{\sigma^{2-\power}C^\power}+2\alpha^{1-1/\power}\sqrt{\sigma^{2-\power}\|\epsilon_1\|^\power}+ 4C^\power\sigma^{1-\power} \alpha^{p-1/\power}+4\alpha^{1-1/\power}\sigma^{1-\power}\|\epsilon_1\|^\power
    \intertext{next, use $\|\epsilon_1\|\le K\sigma$:}
    &\le (1-\alpha)^t \|\epsilon_1\| +(7+2K^{\power/2} + 4K^\power)\sigma\alpha^{1-1/\power} +2\alpha^{\frac{1+p}{2}-1/\power}\sqrt{\sigma^{2-\power}C^\power}+ 4C^\power \sigma^{1-\power}\alpha^{p-1/\power}\\
    &= (1-\alpha)^t \|\epsilon_1\| +(7+2K^{\power/2} + 4K^\power + 2\alpha^{\frac{\power-1}{2}}\sqrt{C^\power\sigma^{-\power}} + 4C^\power\sigma^{-\power}\alpha^{\power -1})\sigma\alpha^{1-1/\power}
\end{align*}
Now, since $p>1$, for any $C\ge 2\sigma(7+2K^{\power/2} + 4K^\power)$ it must hold that for sufficiently small $\alpha$,
\begin{align}
    (7+2K^{\power/2} + 4K^\power + 2\alpha^{\frac{\power-1}{2}}\sqrt{C^\power\sigma^{-\power}} + 4C^\power\sigma^{-\power}\alpha^{\power -1})\sigma\le C\label{eqn:C}
\end{align}
which completes the induction. Therefore we have:
\begin{align*}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t \|\epsilon_1\| + C\alpha^{1-1/\power}
\end{align*}
From which we obtain:
\begin{align*}
    \sum_{t=1}^T \|\hat\epsilon_t\|&\le \frac{\|\epsilon_1\|}{\alpha} + CT\alpha^{1-1/\power}
    \intertext{Set $\alpha = \frac{M}{T^{\frac{\power}{3\power -2}}}$ for sufficiently small $M$ to ensure (\ref{eqn:C}):}
    &\le \frac{\|\epsilon_1\|}{M}T^{\frac{\power}{3\power-2}} + CM^{1-1/\power} T^{\frac{4\power -3}{3\power-2}}
\end{align*}


Thus, overall using the definitions of $\eta$ and Lemma 2 of \cite{cutkosky2020momentum}, we obtain the desired result.

However, all this was assuming that we index $t=1$ at the last reset. Let us now show that the number of resets will be small, and that each reset happens quickly.

First, suppose we perform a reset a some index $t$. We will show that if $\|\hat\epsilon_t\|\le K\sigma$, then with probability at least $1-\delta$, we will never reset again. To see this, we need to understand the probability that $s_t=1$. From Markov inequality,
\begin{align*}
    P[s_t=0]&\le \frac{\E[\power \|\bg_t - \nabla F(\w_t)\|^\power + \power \|\bm_t - \nabla F(\w_t)\|^\power]}{\gamma^\power}\\
    &\le \frac{\power\sigma^\power + \power^2(1-\alpha)^{t\power}\|\hat\epsilon_1\|^\power + \power^2C^\power\alpha^{\power-1}}{\gamma^\power}\\
    &\le D\frac{\sigma^\power}{\gamma^\power}
\end{align*}
for appropriately defined constant $D$. Note that $D$ does not depend on $\sigma$, although it may depend on $K$. Thus for $\gamma$ large enough, we have $P[s_t=0]\le \frac{1}{4}$. This means that with probability at least $1-\delta$, for all $t$:
\begin{align*}
    \frac{1}{t}\sum_{\tau=1}^t s_\tau \ge \frac{3}{4}-\sqrt{\log(T/\delta) t}
\end{align*}
Therefore, if this check ever fails, we must have had $\|\hat\epsilon_t\|\ge K\sigma$. Notice that by Markov inequality, $\|\hat\epsilon_t\|\ge K\sigma$ with probability at most $\frac{1}{K^\power}$, so that with probability at least $1-2\delta$, we reset at most $\log(1/\delta)/\log(K^\power)$ times.


Now, we need to show that, so long as $\|\hat\epsilon\|\ge K\sigma$, we will in fact hit a reset fairly quickly.
TODO HERE FINISH PROOF
\end{proof}


\section{Finding a ``Reasonable'' Starting Gradient}
Given a stream of random variable $x_1,x_2,\dots$, we want to use a small number $N$ of samples in order to find an estimate $\hat x$ such that with probability at least $1-\delta$, $\|\hat x - \E[x]\|=O(\sigma)$, where $\E[\|x-\E[x]\|^\power]\le \sigma^\power$ and we consider $N$ small if $N=O(\log(1/\delta)^2)$.

Our strategy is as follows: by Markov inequality, with probability at least $3/4$, any given sample $x$ is with $O(\sigma)$ of $\E[x]$. Thus we will pick some sample $x_1$, and set $\hat x=x_1$. Then we will look at some more samples $x_2,\dots$ and check for each of them if they are within $O(\sigma)$ of $\hat x$. If $\hat x$ is NOT within $O(\sigma)$ of $\E[x]$, then we would expect the probability that any other $x_i$ is within some appropriate $O(\sigma)$ of $\hat x$ to be smaller than some constant, say $1/4$. Conversely, if $\hat x$ is close to $\E[x]$, then we expect $x_i$ to be close to $\hat x$ with some probability at least say $1/2$. Thus by Hoeffding bound, with high probability we can detect which of these cases is occuring with $O(\log(1/\delta))$ samples. If $\hat x$ is not close to $\E[x]$, we start over with a new $\hat x$. 

==> old_statistics.tex <==

\section{Bounds on Averages of Heavy-Tailed variables}
First, a basic fact about tail bounds and expectations. This should probably be well-known to any sufficiently educated person, but embarrassingly I was not sure about it so I prove it below:
\begin{Proposition}\label{prop:integrate}
Suppose $X$ is a real-valued random variable such that $X\ge 0$ with probability 1. Suppose $B(\delta)$ is such that with probability at least $1-\delta$, $X\le B(\delta)$. Then:
\begin{align*}
    \E[X]\le \int_{0}^1 B(\delta)\ d\delta
\end{align*}
\end{Proposition}
\begin{proof}

Let $F$ be the cumulative distribution function for $X$. Let $\hat F(x)=1-F(x)$. Then by definition we have $1-\hat F(x)$ is the probability that $X\le x$, so we must have $B(\delta) \ge \hat F^{-1}(\delta)$. Then
\begin{align*}
    \E[X] &= \int_{0}^\infty X dF\\
    &=-\int_{0}^\infty X d\hat F
    \intertext{setting $\delta=\hat F(x)$:}
    &=-\int_{1}^0 \hat F^{-1}(\delta) d\delta\\
    &=\int_0^1 \hat F^{-1}(\delta) \ d\delta\\
    &\le \int_0^1 B(\delta)\ d\delta
\end{align*}
\end{proof}

Next, we provide the main result of this section, which bounds the deviation of sums of heavy-tailed quantities from their mean.

The proof of this Lemma follows that of the similar Lemma 3 in \cite{bubeck2013bandits}, generalizing the argument in appropriate places:
\begin{Lemma}
Suppose $X_1,\dots,X_T$ are random variables with means $\mu_1,\dots,\mu_T$ such that $\E[\|X_t-\mu_t\|^{\power}\|]\le \sigma_t^\power$ for some $\sigma_t$ for all $t$ for some $\power\in(1,2]$ and $\sigma_\power\ge 0$. Then for positive numbers $b_1,\dots,b_T$ and any $\delta\in(0,1)$, with probability at least $1-\delta$,
\begin{align*}
    \left\|\sum_{t=1}^T b_t X_t - \sum_{t=1}^T b_t \mu_t\right\|\le \frac{\left(5\sum_{t=1}^T \sigma_t^\power b_t^\power\right)^{1/\power}}{(2\delta)^{1/\power}}
\end{align*}
Furthermore,
\begin{align*}
    \E\left[\left\|\sum_{t=1}^T b_t X_t - \sum_{t=1}^T b_t \mu_t\right\|\right]\le \frac{\power\left(5\sum_{t=1}^T \sigma_t^\power b_t^\power\right)^{1/\power}}{(\power-1)2^{1/\power}}
\end{align*}
\end{Lemma}
\begin{proof}
We will bound the probability:
\begin{align*}
    P\left[\left\|\sum_{t=1}^T b_t X_t - \sum_{t=1}^T b_t \mu_t\right\|\ge \eta\right]
\end{align*}
Notice that for any $c$, this probability is bounded by:
\begin{align}
    P\left[ \|b_t(X_t-\mu_t)\|\ge c\text{ for some }t\right] + P\left[ \left\|\sum_{t=1}^T b_t (X_t -\mu_t)I[\|b_t(X_t-\mu_t)\|\le c]\right\|\ge \eta\right]\label{eqn:sum}
\end{align}
Now, by Markov inequality, for any $t$ we have:
\begin{align*}
    P[\|b_t(X_t - \mu_t)\|\ge c]=P[\|X_t-\mu_t\|^\power \ge \frac{c^\power}{b_t^\power}]\le \frac{ \sigma_t^\power b_t^\power}{c^\power}
\end{align*}
Therefore, by union bound, the first probability term in (\ref{eqn:sum}) is bounded by:
\begin{align*}
    \frac{ \sum_{t=1}^T \sigma_t^\power b_t^\power}{c^\power}
\end{align*}

To make the algebra a little more manageable, let $Z_t = (X_t-\mu_t)I[\|b_t(X_t-\mu_t)\|\le c]$. Then for the second term of (\ref{eqn:sum}), by Chebychev inequality we have:
\begin{align*}
    P&\left[ \left\|\sum_{t=1}^T b_t (X_t -\mu_t)I[\|b_t(X_t-\mu_t)\le c\|]\right\|\ge \eta\right]\\
    &\le \frac{\E\left[ \left\|\sum_{t=1}^T b_tZ_t\right\|^2\right]}{\eta^2}\\
    &\le \frac{\E\left[\sum_{t=1}^Tb_t^2\|Z_t\|^2\right]}{\eta^2}+\frac{\sum_{t\ne t'\in[T]}E\left[ \langle b_t Z_t,b_{t'}Z_{t'}\rangle\right]}{\eta^2}
    \intertext{Using $b_tZ_t$ and $b_{t'}Z_{t'}$ are independent for $t\ne t'$:}
    &\le \frac{\E\left[\sum_{t=1}^Tb_t^2\|Z_t\|^2\right]}{\eta^2}+\frac{\sum_{t\ne t'\in[T]} \langle\E[b_t Z_t],\E[b_{t'}Z_{t'}]\rangle}{\eta^2}\\
    &\le \frac{\E\left[\sum_{t=1}^Tb_t^2\|Z_t\|^2\right]}{\eta^2}+\frac{\sum_{t\ne t'\in[T]} \|\E[b_t Z_t]\|\|\E[b_{t'}Z_{t'}]\|}{\eta^2}
    \intertext{Using the fact that $\power \le 2$ and $\|Z_t\|\le c/b_t$ with probability 1:}
    &\le \frac{\E\left[\sum_{t=1}^Tb_t^2\|Z_t\|^{\power}\left(\frac{c}{b_t}\right)^{2-\power}\right]}{\eta^2}+\frac{\sum_{t\ne t'\in[T]} \|\E[b_t Z_t]\|\|\E[b_{t'}Z_{t'}]\|}{\eta^2}
    \intertext{Now, using $\|Z_t\|\le \|X_t-\mu_t\|$ with probability 1:}
    &\le \frac{\E\left[\sum_{t=1}^Tb_t^\power\|X_t-\mu_t\|^{\power}c^{2-\power}\right]}{\eta^2}+\frac{\sum_{t\ne t'\in[T]} \|\E[b_t Z_t]\|\|\E[b_{t'}Z_{t'}]\|}{\eta^2}\\
    &\le \frac{\sum_{t=1}^Tb_t^\power\sigma_t^\power c^{2-\power}}{\eta^2}+\frac{\sum_{t\ne t'\in[T]} \|\E[b_t Z_t]\|\|\E[b_{t'}Z_{t'}]\|}{\eta^2}
\end{align*}
Now we need to analyze $\|\E[b_tZ_t]\|$. Let us expand out the definition of $Z_t$, so that we are bounding $\|\E[b_t(X_t-\mu_t)I[\|b_t(X_t-\mu_t)\|\le c]]$. Next, notice that:
\begin{align*}
    \E[b_t(X_t-\mu_t)I[\|b_t(X_t-\mu_t)\|\le c] + \E[b_t(X_t-\mu_t)I[\|b_t(X_t-\mu_t)\|> c]= \E[b_t(X_t-\mu_t)]=0
\end{align*}
so that we have:
\begin{align*}
    \|\E[b_tZ_t]\|=\|-\E[b_t(X_t-\mu_t)I[\|b_t(X_t-\mu_t)\|> c]\|\le b_t\E[\|X_t-\mu_t\|I[\|b_t(X_t-\mu_t)\|> c]
\end{align*}
Now, by H\"older inequality with $p=\power$ and $q=\frac{\power}{\power-1}$, we have that 
\begin{align*}
    \|\E[b_t Z_t]\|&\le b_t\E[ \|X_t-\mu_t\|^\power]^{1/\power}\E[I[\|b_t(X_t-\mu_t)\|> c]]^{\frac{\power-1}{\power}}\\
    &=b_t\E[ \|X_t-\mu_t\|^\power]^{1/\power}P[\|b_t(X_t-\mu_t)\|> c]^{\frac{\power-1}{\power}}\\
    &\le b_t\E[ \|X_t-\mu_t\|^\power]^{1/\power}\left(\frac{\sigma_t^\power b_t^\power}{c^\power}\right)^{\frac{\power-1}{\power}}\\
    &\le b_t^\power \sigma_t^\power c^{1-\power}
\end{align*}
Bounding the sum then yields:
\begin{align*}
    \frac{\sum_{t\ne t'\in[T]} \|\E[b_t Z_t]\|\|\E[b_{t'}Z_{t'}]\|}{\eta^2}&\le \frac{\sum_{t\ne t'\in[T]}  b_t^\power \sigma_t^\power c^{1-\power} b_{t'}^\power \sigma_{t'}^\power c^{1-\power}}{\eta^2}\\
    &\le \frac{\left(\sum_{t=1}^T  b_t^\power \sigma_t^\power c^{1-\power}\right)^2}{\eta^2}
\end{align*}
Thus, putting everything together, we have shown:
\begin{align*}
    P&\left[\left\|\sum_{t=1}^T b_t X_t - \sum_{t=1}^T b_t \mu_t\right\|\ge \eta\right]\\
    &\le  \frac{ \sum_{t=1}^T \sigma_t^\power b_t^\power}{c^\power} + \frac{\sum_{t=1}^Tb_t^\power\sigma_t^\power c^{2-\power}}{\eta^2} + \frac{\left(\sum_{t=1}^T  b_t^\power \sigma_t^\power c^{1-\power}\right)^2}{\eta^2}
    \intertext{Now, set $c=\eta$:}
    &=2\frac{ \sum_{t=1}^T \sigma_t^\power b_t^\power}{\eta^\power} + \frac{\left(\sum_{t=1}^T  b_t^\power \sigma_t^\power\right)^2}{\eta^{2\power}}
\end{align*}

Now, notice that if $\frac{ \sum_{t=1}^T \sigma_t^\power b_t^\power}{\eta^\power}\ge 1/2$, then the above bound is larger than 1, so we tighten the bound to:
\begin{align*}
    P&\left[\left\|\sum_{t=1}^T b_t X_t - \sum_{t=1}^T b_t \mu_t\right\|\ge \eta\right]\\
&\le \frac{5 \sum_{t=1}^T \sigma_t^\power b_t^\power}{2\eta^\power}
\end{align*}
Now set $\delta =  \frac{ \sum_{t=1}^T \sigma_t^\power b_t^\power}{2\eta^\power} $ and solve for $\eta$ to conclude the first result of the Lemma.

For the second result, simply apply Proposition \ref{prop:integrate} and integrate the probability bound from $\delta=0$ to $1$.
\end{proof}

\section{Streaming and Translation-invariant high-probability mean estimates}

In this section we provide a method for maintaining a high-probability mean estimate for a stream of heavy-tailed variables $X_1,X_2,\dots,X_T$ with mean $\mu$. The method will have $O(1)$ memory overhead, and take $O(1)$ time for each element of the stream. The basic idea is as follows: if we are provided with an ``anchor point'' $Z$ such that $\|Z-\mu\|=O(\sigma)$, then given a new sample $X_t$, we can replace $X_t$ with a version that has been clipped towards $Z$:
\begin{align}
   \hat X_t= Z + (X_t- Z) \frac{\min(\|X_t-Z\|, \tau)}{\|X_t - Z\|} \label{eqn:clip}
\end{align}
for some threshold $\tau$. Then we can show that:
\begin{align*}
   \| \E[\hat X_t] - \mu\|\le O\left(\frac{\sigma^\power + \|Z-\mu\|^\power}{\tau^{\power-1}}\right)= O\left(\frac{\sigma^\power}{\tau^{\power-1}}\right)
\end{align*}
Further,
\begin{align*}
    \E[\|\hat X_t - \E[\hat X_t]\|^2]&\le O((\sigma^\power + \|Z-\mu\|^\power)\tau^{2-\power})
\end{align*}
Moreover, it is clear that $\hat X_t$ is $\tau$-subgaussian since it lies within a ball of radius $\tau$. Therefore, by some kind of Bernstein or Bennett inequality, we have with probability at least $1-\delta$
\begin{align*}
    \left\|\frac{1}{T}\sum_{t=1}^T \hat X_t- \mu\right\|\le O\left(\frac{\sigma^\power}{\tau^{\power-1}} + \sqrt{\frac{\tau^{2-\power}\sigma^{\power}\log(1/\delta)}{T}}+ \tau \frac{\log(1/\delta)}{T}\right)
\end{align*}
Now set $\tau = \sigma T^{1/\power}/\log^{1/\power}(1/\delta)$ to obtain with probability at least $1-\delta$:
\begin{align*}
    \left\|\frac{1}{T}\sum_{t=1}^T \hat X_t- \mu\right\|\le O\left[\sigma\left(\frac{\log(1/\delta)}{T}\right)^{\frac{\power-1}{\power}}\right]  
\end{align*}

But how do we get the good anchor value $Z$? One approach is to simply draw a sample $X$ and set that to be $Z$. With probability at least say $\frac{3}{4}$, this sample will be close enough to $\mu$. However, this leaves a $\frac{1}{4}$ failure chance. Instead, we will have a method for quickly detecting such failures. Specifically, as we process samples $X_t$, we will record the frequency of the event $\|X_t - Z\|\le k$ for some particular threshold $k$. By standard concentration, after some $B$ iterations thiss frequency will be within roughly $\frac{1}{\sqrt{B}}$ of the true probability of this event. We will argue that the true probability is high if $Z$ is close to $\mu$, and low otherwise. Thus If this frequency every dips too low, we can conclude that our chosen value of $Z$ is poor, and start again. We will only need to restart logarithmically many times, and each failed $Z$ can be detected quickly since it turns out $B$ does not need to be very large.

We will need the following technical Lemma:
\begin{Lemma}\label{thm:threshbound}
Suppose $X$ is a random variable such that $\E[\|X-\mu\|^\power]\le \sigma^\power$. Let be $Z$ be any other value. Let $p=P[\|X-Z\|\le k]$ for some $k$. Then:
\begin{align*}
    k - \frac{\sigma}{(1-p)^{1/\power}} \le \|Z-\mu\|\le k + \frac{\sigma}{p^{1/\power}}
\end{align*}
\end{Lemma}
\begin{proof}
By triangle inequality, we have:
\begin{align*}
    p=P[\|X-Z\|\le k]\le P[\|Z-\mu\| - \|X-\mu\|\le k]
\end{align*}
Therefore by Markov inequality,
\begin{align*}
    p&\le P[\|X-\mu\|\ge \|Z-\mu\|-k]\\
    &\le \frac{\sigma^\power}{(\|Z-\mu\|-k)^\power}
    \intertext{solving for $\|Z-\mu\|$:}
    \|Z-\mu\|&\le k + \frac{\sigma}{p^{1/\power}}
\end{align*}
For the lower bound, we have again by triangle inequality:
\begin{align*}
    P[ \|X-Z\|>k] \le P[\|X-\mu\|+\|Z-\mu\|>k]=P[\|X-\mu\|>k-\|Z-\mu\|]
\end{align*}
Therefore:
\begin{align*}
    1-p&=P[\|X-\mu\|>k]\\
    &\le P[\|X-\mu\|>k-\|Z-\mu\|]\\
    &\le \frac{\sigma^\power}{(k-\|Z-\mu\|)^{\power}}\\
    \|Z-\mu\|&\ge k-\frac{ \sigma}{(1-p)^{1/\power}}
\end{align*}
\end{proof}


\begin{Lemma}\label{thm:threshold}
Suppose $X_1,\dots,X_T$ are random vectors with means $\mu_1,\dots,\mu_T$. Suppose there is some $\power\in(1,2]$ such that for all $t$ there is some $\sigma_t<\infty$ such that $\E[\|X_t-\mu_t\|^\power]\le \sigma_t^\power$. Let $Z_1,\dots,Z_T$ be some other set of random vectors such that $Z_t$ is independent of $X_t,\dots,X_T$ for all $t$. For some $\tau>0$, let $\hat X_t = Z_t + \frac{X_t - Z_t}{\|X_t-Z_t\|}\min(\tau, \|X_t-Z_t\|)$. Then with probability at least $1-\delta$:
\begin{align*}
    \left\|\sum_{t=1}^T \hat X_t - \mu_t\right\|&\le \frac{4\tau}{3}\log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right] + \sqrt{2 \log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right]\sum_{t=1}^T 2^{\power-1}(\sigma_t^\power +\|Z_t-\mu_t\|^\power)\tau^{2-\power}}\\
    &+ \frac{2\tau}{3} + \sqrt{\sum_{t=1}^T 2^{\power-1}(\sigma_t^\power +\|Z_t-\mu_t\|^\power)\tau^{2-\power}}+\sum_{t=1}^T\frac{2^{\power-1}\sigma_t^\power + 2^{\power-1}\|Z_t-\mu_t\|^\power}{\tau^{\power-1}}
\end{align*}
Further, if $\|Z_t - \mu_t\|\le C\sigma_t$ for some $C$ for all $t$, then with
\begin{align*}
    \tau^\power = \sum_{t=1}^T\sigma_t^\power
\end{align*}
we have:
\begin{align*}
    \left\|\sum_{t=1}^T \hat X_t - \mu_t\right\|&\le \left[4 + 2^{\power+1}(1+C)\right]\left(\sum_{t=1}^T \sigma_t^\power\right)^{\frac{1}{\power}}\log\left[ \frac{50}{\delta}\left(\frac{T}{\left(\sum_{t=1}^T \sigma_t^\power\right)^{1/\power}}+3\right)\right]
\end{align*}
(NOTE better dependencies on the log power can be gotten by tuning $\tau$ better, but then the bound won't hold for any $\delta$ in hindsight...).
\end{Lemma}
\begin{proof}
First, we will bound $\|\E[\hat X_t] - \mu_t\|$, following analysis similar to that present in \cite{zhang2019adam}:
\begin{align*}
    \|\E[\hat X_t] - \mu_t\|&=\|\E[\hat X_t -X_t]\|\\
    &=\|\E[(\hat X_t -Z_t) - (X_t - Z_t)]\|\\
    &\le \E[\|(\hat X_t -Z_t) - (X_t - Z_t)\|]\\
    &\le \E[\|X_t-Z_t\|\one[\|X_t-Z_t\|\ge \tau]]\\
    &\le \E[\|X_t-Z_t\|^\power/\tau^{\power-1}]\\
    &\le \E[(\|X_t-\mu_t\|+\|Z_t-\mu_t\|)^\power/\tau^{\power-1}]\\
    &\le \frac{2^{\power-1}\sigma_t^\power + 2^{\power-1}\|Z_t-\mu_t\|^\power}{\tau^{\power-1}}
\end{align*}
where the last line follows from Jensen inequality and $\power>1$.

Next, we bound the variance $\E[\|\hat X_t - \E[\hat X_t]\|^2]$:
\begin{align*}
    \E[\|\hat X_t - \E[\hat X_t]\|^2]&\le \E[\|\hat X_t -Z_t\|^2]\\
    &\le \E[\|X_t - Z_t\|^\power \tau^{2-\power}]\\
    &\le \E[2^{\power-1}(\|X_t - \mu_t\|^\power +\|Z_t -\mu_t\|^\power)\tau^{2-\power}]\\
    &\le 2^{\power-1}(\sigma_t^\power +\|Z_t-\mu_t\|^\power)\tau^{2-\power}
\end{align*}

Now, invoke Proposition \ref{thm:bernstein}, observing that $\|\hat X_t - Z_t\|\le \tau$ always so that $\|\hat X_t - \E[\hat X_t]\|\le 2\tau$. With probability $1-\delta$:

\begin{align*}
    \left\|\sum_{t=1}^T \hat X_t - \E[\hat X_t]\right\|&\le \frac{4\tau}{3}\log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right] + \sqrt{2 \log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right]\sum_{t=1}^T 2^{\power-1}(\sigma_t^\power +\|Z_t-\mu_t\|^\power)\tau^{2-\power}}\\
    &\quad\quad + \frac{2\tau}{3} + \sqrt{\sum_{t=1}^T 2^{\power-1}(\sigma_t^\power +\|Z_t-\mu_t\|^\power)\tau^{2-\power}}
\end{align*}
Therefore by triangle inequality:
\begin{align*}
    \left\|\sum_{t=1}^T \hat X_t - \mu_t\right\|&\le \frac{4\tau}{3}\log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right] + \sqrt{2 \log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right]\sum_{t=1}^T 2^{\power-1}(\sigma_t^\power +\|Z_t-\mu_t\|^\power)\tau^{2-\power}}\\
    &+ \frac{2\tau}{3} + \sqrt{\sum_{t=1}^T 2^{\power-1}(\sigma_t^\power +\|Z_t-\mu_t\|^\power)\tau^{2-\power}}+\sum_{t=1}^T\frac{2^{\power-1}\sigma_t^\power + 2^{\power-1}\|Z_t-\mu_t\|^\power}{\tau^{\power-1}}
\end{align*}

This proves the first statement of the Lemma. Now if we assume $\|Z_t -\mu_t\|^\power \le C\sigma_t^\power$ for all $t$, this becomes:
\begin{align*}
    \left\|\sum_{t=1}^T \hat X_t - \mu_t\right\|&\le \frac{4\tau}{3}\log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right] + \sqrt{2 \log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right]\sum_{t=1}^T 2^{\power-1}(1+C)\sigma_t^\power\tau^{2-\power}}\\
    & +\frac{2\tau}{3} + \sqrt{\sum_{t=1}^T 2^{\power-1}(1+C)\sigma_t^\power \tau^{2-\power}}+\sum_{t=1}^T\frac{2^{\power-1}(1+C)\sigma_t^\power}{\tau^{\power-1}}
\end{align*}
% Now with (note this is an implicit equation... can make explicit with some maxes later)
% \begin{align*}
%     \tau^\power = \sum_{t=1}^T\frac{\sigma_t^\power}{\log\left[ \frac{50}{\delta}\left(\frac{T}{\tau} + 1\right)\right]}
% \end{align*}
% we obtain:
% \begin{align*}
%     \left\|\sum_{t=1}^T \hat X_t - \mu_t\right\|&\le \left[3 + 2^{\power-1}(1+C)\right]\left(\sum_{t=1}^T \sigma_t^\power\right)^{\frac{1}{\power}}\left(\log\left[ \frac{50}{\delta}\left(\frac{T}{\tau}+1\right)\right]\right)^{\max\left(\frac{1}{\power},\frac{\power-1}{\power}\right)}
% \end{align*}

Now, with
\begin{align*}
    \tau^\power = \sum_{t=1}^T\sigma_t^\power
\end{align*}
we have simultaneously for all $\delta\in(0,1)$, with probability at least $1-\delta$:
\begin{align*}
    \left\|\sum_{t=1}^T \hat X_t - \mu_t\right\|&\le \left[4 + 2^{\power+1}(1+C)\right]\left(\sum_{t=1}^T \sigma_t^\power\right)^{\frac{1}{\power}}\log\left[ \frac{50}{\delta}\left(\frac{T}{\tau}+3\right)\right]
\end{align*}
\end{proof}



The following is a kind of vector Bernstein inequality, adapted from \cite{minsker2011some} Theorem 3.2:
\begin{Proposition}\label{thm:bernstein}
Suppose $X_1,\dots,X_T$ are random vectors in a $d$-dimensional space such $X_t-\mu_t$ form a martingale difference sequence satisfying $\E[\|X_t-\mu_t\|^2|X_1,\dots,X_{t-1}]\le \sigma^2_t$ for some $\sigma_1,\dots,\sigma_T$. Further, suppose $\|X_t-\mu_t\|\le D$ with probability 1. Then for any non-negative scalars $b_1,\dots,b_T$, for any $\eta\ge\frac{1}{6}\left( D+ \sqrt{D^2 +36\sum_{t=1}^T \sigma_t^2}\right)$:
\begin{align*}
    P\left[\left\|\sum_{t=1}^T b_t X_t - b_t\mu_t\right\|\ge \eta\right]\le 50\left(\frac{2T}{D} + 1\right)\exp\left[-\frac{\eta^2/2}{\eta D/3+\sum_{t=1}^T b_t^2\sigma_t^2}\right]
\end{align*}
And further, for any $\delta\in [0,1]$, with probability at least $1-\delta$:
\begin{align*}
    \left\|\sum_{t=1}^T b_t X_t - b_t\mu_t\right\|&\le \frac{2D}{3}\log\left[ \frac{50}{\delta}\left(\frac{2T}{D} + 1\right)\right] + \sqrt{2 \log\left[ \frac{50}{\delta}\left(\frac{2T}{D} + 1\right)\right]\sum_{t=1}^T b_t^2\sigma_t^2}\\
    &\quad\quad + \frac{1}{6}\left( D+ \sqrt{D^2 +36\sum_{t=1}^T \sigma_t^2}\right)
\end{align*}
\end{Proposition}



The following is a better vector Bernstein inequality, adapted from \cite{tropp2015introduction} Theorem 7.3.1:
\begin{Proposition}\label{thm:bernstein}
Suppose $X_1,\dots,X_T$ are random vectors in a $d$-dimensional space such $X_t-\mu_t$ form a martingale difference sequence satisfying $\E[\|X_t-\mu_t\|^2|X_1,\dots,X_{t-1}]\le \sigma^2_t$ for some $\sigma_1,\dots,\sigma_T$. Further, suppose $\|X_t-\mu_t\|\le D$ with probability 1. Then for any non-negative scalars $b_1,\dots,b_T$, for any $\eta\ge\frac{1}{6}\left( D+ \sqrt{D^2 +36\sum_{t=1}^T \sigma_t^2}\right)$:
\begin{align*}
    P\left[\left\|\sum_{t=1}^T b_t X_t - b_t\mu_t\right\|\ge \eta\right]\le 50\left(\frac{2T}{D} + 1\right)\exp\left[-\frac{\eta^2/2}{\eta D/3+\sum_{t=1}^T b_t^2\sigma_t^2}\right]
\end{align*}
And further, for any $\delta\in [0,1]$, with probability at least $1-\delta$:
\begin{align*}
    \left\|\sum_{t=1}^T b_t X_t - b_t\mu_t\right\|&\le \frac{2D}{3}\log\left[ \frac{50}{\delta}\left(\frac{2T}{D} + 1\right)\right] + \sqrt{2 \log\left[ \frac{50}{\delta}\left(\frac{2T}{D} + 1\right)\right]\sum_{t=1}^T b_t^2\sigma_t^2}\\
    &\quad\quad + \frac{1}{6}\left( D+ \sqrt{D^2 +36\sum_{t=1}^T \sigma_t^2}\right)
\end{align*}
\end{Proposition}



==> sgd.tex <==
\section{Normalized SGD with Momentum}\label{sec:normalized}
In this section, we describe our algorithms for finding critical points with high probability in non-convex objectives. Our analysis makes use of gradient clipping, momentum, and normalized updates. Clipping is a standard technique for mitigating the effect of heavy tails, essentially by throwing out outlier data. Momentum is useful as it intuitively averages together many clipped gradients, resulting in a gradient estimate that concentrates about its mean with high probability. Normalizing the updates allows for significantly simplified analyses because the bias terms introduced by the moving average in momentum are now very precisely controlled by the learning rate, as originally analyzed in \cite{cutkosky2020momentum}.
\begin{algorithm}
   \caption{Normalized SGD with Clipping and Momentum}
   \label{alg:nsgdclip}
   \begin{algorithmic}
      \STATE{\bfseries Input: } Initial Point $\bw_1$, learning rates $\eta$, momentum parameters $\alpha$, clipping parameter $\tau$, time horizon $T$:
      \STATE Set $\bm_1 = 0$.
      \FOR{$t=1\dots T$}
      \STATE Sample $z_t\sim P_z$.
      \STATE Set $\bgclip_t = \frac{\nabla f(\bw_t, z_t)}{\|\nabla f(\bw_t, z_t)\|}\min(\tau, \|\nabla f(\bw_1,z_t)\|)$.
      \STATE Set $\bm_t = \beta \bm_{t-1}+ (1-\beta) \bgclip_t$.
      \STATE Set $\bw_{t+1} = \bx_t  - \eta \frac{\bm_t}{\|\bm_t\|}$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}



\begin{restatable}{Theorem}{thmnsgdclip}\label{thm:nsgdclip}
Suppose $\E_z[\|\nabla f(\bw,z)-\nabla F(\bx)\|^\power]\le G^\power$ for all $\bx$ for some $G$. Suppose $F$ is $L$-smooth. Set $\beta=1-\alpha$, $\alpha = \frac{b}{T^{\frac{\power}{3\power-2}}}$ and $\eta = \frac{c}{T^{\frac{2\power -1}{3\power-2}}}$ for arbitrary constant $b$ and $c$ satisfying $\alpha \le 1$ and set $\tau=G/\alpha^{1/\power}$. Then with probability at least $1-\delta$:
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|&\le  O\left(\frac{\log(T/\delta)}{T^{\frac{\power-1}{3\power-2}}}\right)
\end{align*}
where the big-Oh hides constant that depend on $L$, $G$ $b$, $c$, and $F(\bw_1)-F(\bw_{T+1})$, but not $T$ or $\delta$.
\end{restatable}
This Theorem provides an analog of the standard in-expectation result for non-convex optimization, but now the result holds with high-probability. Note that this matches the in-expectation convergence rates from \cite{zhang2020adaptive}. The next Theorem takes this theme one step further: it shows that after a brief ``burn-in'' period, the decrease in objective value will in fact be \emph{monotonic} with high probability:
\begin{restatable}{Theorem}{thmnsgdclipburnin}\label{thm:nsgdclipburnin}
Under the assumptions of Theorem \ref{thm:nsgdclip}, define the constants:
\begin{align*}
K&=6\max(1,\log(3T/\delta)) + 3\max(1,\log(3T/\delta)) + 1\\
    Z&= \frac{cL}{b}+GKb^{\frac{\power-1}{\power}}
\end{align*}
Then, with probability at least $1-\delta$, if
\begin{align*}
t\ge \mathcal{T}=\frac{T^\frac{\power}{3\power-2}}{b}\left(\frac{\power-1}{3\power-2}\log(T) +\log(G)- \log(Z)\right)
\end{align*}
Then we have
\begin{align*}
    \|\bm_t-\nabla F(\bw_t)\|&\le\frac{2Z}{T^{\frac{\power-1}{3\power-2}}}
\end{align*}
And so long as
\begin{align}
\|\bm_t\|\ge 2\left(\frac{22 Z}{T^{\frac{\power-1}{3\power-2}}} + \frac{3Lc}{2T^{\frac{2\power-1}{3\power-2}}}\right)\label{eqn:mcondition}
\end{align}
we have $F(\bw_{t+1})< F(\bw_t)-\frac{\eta}{2}\|\bm_t\|$. Moreover, if (\ref{eqn:mcondition}) is ever not satisfied, we must have 
\begin{align*}
    \|\nabla F(\bw_t)\|\le \frac{46 Z}{T^{\frac{\power-1}{3\power-2}}} + \frac{6Lc}{2T^{\frac{2\power-1}{3\power-2}}}
\end{align*}
Finally, if $t$ is the iteration with smallest value of $\|\bm_t\|$ such that $t\ge \mathcal{T}$, we have with probability at least $1-\delta$:
\begin{align*}
\|\nabla F(\bw_t)\| \le O\left(\frac{\log(T/\delta)}{T^{\frac{\power-1}{3\power-2}}}\right)
\end{align*}
\end{restatable}

Theorem \ref{thm:nsgdclipburnin} shows that after a small burn-in period $\mathcal{T}=o(T)$, $\bm_t$ is very likely to be an extremely good estimate of the true gradient $\nabla F(\bx_t)$. Moreover, we can empirically detect this event by monitoring the norm of the exponentially weighted moving average $\bm$. This burn-in period is especially interesting given the success of learning rate schedules that incorporate a ``warm-up'' component, in which the learning rate actually increases during the first iterations. Our result seems to hint at a mechanism for this schedule: by keeping the learning rate small during the burn-in period, we can limit any increase in the objective value until we reach the stage at which it begins to decrease steadily.

Further, Theorem \ref{thm:nsgdclipburnin} provides a very concrete algorithm to find critical points: after the burn-in period of $\tilde O(T^{\frac{\power}{3\power-2}})$ iterates, we can simply return the point $\bx_t$ with the smallest value of $\|\bm_t\|$. Intuitively, this works because the objective value can only increase by a total of $O(T^{\frac{\power}{3\power-2}}\eta)=O(T^{\frac{1-\power}{3\power-2}})=O(1)$ during the burn-in period so even without a learning rate ``warm-up'', we should not expect the burn-in period to have too significant an effect on the objective value. After the burnin-in period, $\bm_t$ is always very close to $\nabla F(\bw_t)$, so we make steady progress until a critical point is encountered.

\begin{proof}[Proof of Theorem \ref{thm:nsgdclip}]
Define $\hat \epsilon_t = \bm_t - \nabla F(\bw_t)$. and $\epsilon_t = \bgclip_t - \nabla F(\bw_t)$. Also, define $S(a,b)=\nabla F(a)-\nabla F(b)$. By smoothness, we have $\|S(\bw_t,\bw_{t+1})\|\le L\|\bw_t-\bw_{t+1}\|$

If we define $\bw_0=\bw_1$, then we have the following recursive formulation for any $t\ge 0$:
\begin{align*}
    \bm_{t+1} &= (1-\alpha) (\nabla F(\bw_t) + \hat \epsilon_t) + \alpha\bg^{\text{ clip}}_{t+1}\\
    &=\nabla F(\bw_{t+1}) + (1-\alpha)(S(\bw_t,\bw_{t+1})+\hat \epsilon_t) + \alpha\epsilon_{t+1}\\
    \hat \epsilon_{t+1}&= (1-\alpha)S(\bw_t,\bw_{t+1})+(1-\alpha)\hat \epsilon_t + \alpha \epsilon_{t+1}
\end{align*}
Now, we unravel the recursion for $t+1$ iterations:
\begin{align*}
    \hat \epsilon_{t+1}&=(1-\alpha)^t\hat \epsilon_0 +\alpha\sum_{t'=0}^{t} (1-\alpha)^{t'} \epsilon_{t+1-t'}\\
    &+ (1-\alpha)\sum_{t'=0}^{t}(1-\alpha)^{t'} S(\bw_{t-t'},\bw_{t+1-t'})
\end{align*}
Next, take the magnitude of both sides and use triangle inequality (using the fact that $\|S(\bw_a,\bw_{t+1})\|\le L\eta$):
\begin{align*}
    &\|\hat \epsilon_{t+1}\|\le (1-\alpha)^t\|\hat\epsilon_0\| +\alpha\left\|\sum_{t'=0}^{t} (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|\\
    &\quad\quad\quad+ (1-\alpha)\eta L \sum_{t'=0}^{t}(1-\alpha)^{t'}\\
    &\quad\le (1-\alpha)^t G + \frac{(1-\alpha)\eta L}{\alpha}+\alpha\left\|\sum_{t'=0}^{t} (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|
\end{align*}
where in the second line we have used $\bm_0=0$ and $\|\nabla F(\bw_0)\|\le G$, which follows since $\|\nabla F(\bw_0)\|\le \E_z[\|\nabla f(\bw_0,z)\|^\power]^{1/\power}=G$.

Now, by Lemma \ref{thm:thresholdsimple}, with probability at least $1-\delta/T$:
\begin{align*}
    &\left\|\sum_{t'=0}^{t} (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|\le  6\tau\max(1,\log(3T/\delta))\\
    &\quad\quad+3\sqrt{\sum_{t'=0}^t(1-\alpha)^{2t'}G^\power \tau^{2-\power}\max(1,\log(3T/\delta))}\\
    &\quad\quad+\sum_{t'=0}^t \frac{(1-\alpha)^{t'}G^\power}{\tau^{\power-1}}\\
    &\le 6\tau\max(1,\log(3T/\delta))+\frac{G^\power}{\alpha \tau^{\power-1}}\\
    &\quad \quad +\frac{3\sqrt{G^\power \tau^{2-\power}\max(1,\log(3T/\delta))}}{\sqrt{\alpha}}
\end{align*}

Therefore, with probability at least $1-\delta/T$:
\begin{align}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t G + \frac{(1-\alpha)\eta L}{\alpha} + 6\alpha\tau\max(1,\log(3T/\delta))\nonumber\\
    &\quad+ 3\sqrt{ \alpha G^\power\tau^{2-\power}\max(1,\log(3T/\delta))}+\frac{G^\power}{ \tau^{\power-1}}\nonumber\\
    % &\quad+\frac{4\tau \alpha}{3}\log\left[\frac{50}{\delta}\left(\frac{T}{\tau}+1\right)\right]+\sqrt{2\alpha\log\left[\frac{50}{\delta}\left(\frac{T}{\tau}+1\right)\right]G^\power \tau^{2-\power}}\\
    % &\quad+\frac{2\tau \alpha}{3} + \sqrt{2^{\power-1}\alpha G^\power \tau^{2-\power}} + \frac{2^{\power-1}G^\power}{ \tau^{\power-1}}
    \intertext{
Now, with $\tau=\frac{G}{\alpha^{1/\power}}$, and $D_\delta=\max(1,\log(3T/\delta))$ this becomes:}
&\le (1-\alpha)^t G + \frac{(1-\alpha)\eta L}{\alpha}\nonumber\\
&\mkern-24mu +G\alpha^{1-1/\power}\left[6D_\delta + 3\sqrt{D_\delta} + 1\right]\nonumber\\
    % \frac{4}{3}\log\left[\frac{50}{\delta}\left(\frac{T\alpha^{1/\power}}{G}+1\right)\right]+\sqrt{2\log\left[\frac{50}{\delta}\left(\frac{T\alpha^{1/\power}}{G}+1\right)\right]}\right.\\
    % &\quad\left.+\frac{2}{3} + \sqrt{2^{\power-1}} + 2^{\power-1}\right]\\
    &=(1-\alpha)^tG+ \frac{(1-\alpha)\eta L}{\alpha} + G\alpha^{1-1/\power}K\label{eqn:hatepsbound}
\end{align}
where we define the constant $K=6D_\delta + 3\sqrt{D_\delta} + 1$. 


Now, we have from \cite{cutkosky2020momentum} Lemma 2:
\begin{align*}
   \sum_{t=1}^T &\|\nabla F(\bw_t)\|\\
   &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+8\sum_{t=1}^T \|\hat\epsilon_t\|
    \intertext{so with probability at least $1-\delta$:}
    &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+8\sum_{t=1}^T(1-\alpha)^tG\\
    &\quad+ \frac{(1-\alpha)\eta L}{\alpha} + G\alpha^{1-1/\power}K\\
    &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+\frac{8G(1-\alpha)}{\alpha} \\
    &\quad+ \frac{(1-\alpha)\eta T L}{\alpha} + GT\alpha^{1-1/\power}K
\end{align*}
Now set $\alpha = \frac{b}{T^{\frac{\power}{3\power-2}}}$ and $\eta = \frac{c}{T^{\frac{2\power -1}{3\power-2}}}$. This yields:
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|&\le  O\left( T^{\frac{1-\power}{3\power-2}}\log(T/\delta)\right)
\end{align*}
\end{proof}

The proof of Theorem \ref{thm:nsgdclipburnin} follows essentially the same idea as that of Theorem \ref{thm:nsgdclip}. However, this time we use the explicit bound on $\|\hat\epsilon_t\|$ and observe that after the burn-in period, the contribution from $\|\epsilon_1\|$ has decreased exponentially to be insignificant, and so $\bm_t$ will be a very high-quality estimate of $\nabla F(\bx_t)$ at every single iteration.

\begin{proof}[Proof of Theorem \ref{thm:nsgdclipburnin}]
Use the settings $\eta=\frac{c}{T^{\frac{2\power-1}{3\power-2}}}$ and $\alpha = \frac{b}{T^{\frac{\power}{3\power-2}}}$ and notice that from equation (\ref{eqn:hatepsbound}) that with probability $1-\delta$, for all $t$:
\begin{align*}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t G + \frac{cL}{bT^{\frac{\power-1}{3\power-2}}}+\frac{GKb^{\frac{\power-1}{\power}}}{T^{\frac{\power-1}{3\power-2}}}\\
    &=(1-\alpha)^t G + \frac{Z}{T^{\frac{\power-1}{3\power-2}}}
\end{align*}
Further, we have
\begin{align*}
    \log(1-\alpha)&\le -\alpha\\
    \log\left(G(1-\alpha)^t)\right) &\le -t\alpha +\log(G)
\end{align*}
Therefore, if $t$ satisfies:
\begin{align*}
    t\ge \frac{T^\frac{\power}{3\power-2}}{b}\left(\frac{\power-1}{3\power-2}\log(T) +\log(G) - \log\left(Z\right)\right)
\end{align*}
we have with probability at least $1-\delta$:
\begin{align*}
\|\hat \epsilon_{t+1}\|&\le \frac{2Z}{T^{\frac{\power-1}{3\power-2}}}
\end{align*}
This implies the bound on $\|\nabla F(\bw_t)\|$ when $\|\bm_t\|$ is smaller than the threshold described in the Theorem statement. Next, again from Lemma 2 of \cite{cutkosky2020momentum},
\begin{align*}
    F(\bw_{t+1})&\le F(\bw_t) - \frac{\eta}{3}\|\nabla F(\bw_t)\| + \frac{8\eta}{3}\|\hat\epsilon_t\| + \frac{L\eta^2}{2}\\
    &\le F(\bw_t) - \frac{\eta}{3}\|\bm_t\| + \frac{11\eta}{3}\|\hat\epsilon_t\| + \frac{L\eta^2}{2}\\
    &\le F(\bw_t) - \frac{\eta}{3}\|\bm_t\| +\frac{\eta}{3}\left(\frac{22Z }{T^{\frac{\power-1}{3\power-2}}} + \frac{3Lc}{2T^{\frac{2\power-1}{3\power-2}}}\right)
\end{align*}
from which we can conclude that if $\|\bm_t\|\ge 2\left(\frac{22Z }{T^{\frac{\power-1}{3\power-2}}} + \frac{3Lc}{2T^{\frac{2\power-1}{3\power-2}}}\right)$, $F(\bw_{t+1})\le F(\bw-t) - \frac{\eta}{6}\|\bm_t\|$.

Now, for the final part of the Theorem, observe that since $F$ is $G$-Lipschitz, we must have that 
\begin{align*}
    F(\bw_{\mathcal{T}})-F(\bw_1)\le G\mathcal{T} \eta=O(\log(T))
\end{align*}
so that $F(\bw_{\mathcal{T}}) - F(\bw_{T+1}) \le O(F(\bw_1)-F(\bw_{T+1}) + \log(T))$. Now consider two cases, either 
\begin{align*}
    \min_{t\ge \mathcal{T}} \|\bm_t\|\le 2\left(\frac{22Z }{T^{\frac{\power-1}{3\power-2}}} + \frac{3Lc}{2T^{\frac{2\power-1}{3\power-2}}}\right)
\end{align*}
or not. In the first case, by our bound on $\|\hat \epsilon_t\|$, the desired bound on $\|\nabla F(\bw_t)\|$ follows. In the latter case, we have
\begin{align*}
     F(\bw_{T+1})&\le F(\bw_{\mathcal{T}})-\frac{\eta}{6}\sum_{t=\mathcal{T}}^T \|\bm_t\|
\end{align*}
So that 
\begin{align*}
    &\min_{t\ge \mathcal{T}} \|\bm_t\| \le O\left(\frac{F(\bw_1)-F(\bw_{T+1}) + \log(T)}{T\eta}\right) \\
    &= \tilde O\left(\frac{1}{T^{\frac{2\power-1}{3\power-2}}}\right)
\end{align*}
And so again the result follows from our bound on $\|\hat\epsilon_t\|$. 
\end{proof}

In addition to providing a method for identifying critical points, Theorem \ref{thm:nsgdclipburnin} also provides an intuitively desirable guarantee about the \emph{last-iterate} of the algorithm $\bw_T$. Specifically, one can easily check that the following Corollary:
\begin{Corollary}\label{thm:lastiterate}
Under the notation and assumptions of Theorem \ref{thm:nsgdclipburnin}, with probability at least $1-\delta$, there exists some $\hat w$ such that both of the following inequalities hold:
\begin{align*}
    \|\nabla F(\hat w)\|&\le O\left(\frac{\log(T/\delta)}{T^{\frac{\power-1}{3\power-2}}}\right)\\
    F(\bw_T) &\le F(\hat w)
\end{align*}
where $\bw_T$ is the last iterate of Algorithm \ref{alg:nsgdclip}
\end{Corollary}
\begin{proof}
Set $\hat w$ to be the last iterate for which condition \ref{eqn:mcondition} does not hold. Then the result is immediately implied by Theorem \ref{thm:nsgdclip}.
\end{proof}

In most applications we are not actually interested in finding critical points, but instead wish to actually minimize the objective $F$. This observation tells us that our objective value is at least never worse than it would have been if had indeed searched specifically for a critical point. Moreover, by providing a guarantee about $\bw_T$, we have a closer match to practical use-cases: many of the theoretical analyses of non-convex stochastic gradient methods \cite{ghadimi2013stochastic, ward2019adagrad,li2019convergence} only show that a \emph{randomly selected iterate} has a small gradient norm. In contrast, Corollary \ref{thm:lastiterate} provides a non-asymptotic guarantee for the final iterate, which is the iterate most likely to be deployed after training in practice.

\section{Second-Order Smooth Losses}\label{sec:igt}
In this section, we provide our extension to losses that are \emph{second order smooth}. The overall method is very similar: we employ normalized SGD with momentum. However, in order to take advantage of the second-order smoothness, we will need to use a more advanced form of momentum. Specifically, we use implicit gradient transport \cite{arnold2019reducing}, as implemented by \cite{cutkosky2020momentum} in the NIGT algorithm. This algorithm replaces the standard momentum update with an extrapolation procedure:
\begin{align*}
    \bm_t = \beta \bm_{t-1} +  (1-\beta) \nabla f\left(\bw_t + \frac{\beta(\bw_t - \bw_{t-1})}{1-\beta}, z_t\right)
\end{align*}
By evaluating the gradient at the ``shifted'' point $\bw_t + \frac{\beta(\bw_t - \bw_{t-1})}{1-\beta}$ and performing a second-order Taylor expansion enabled by the second-order smoothness assumption, it is possible to show that $\bm_t$ is a less-biased estimate of $\nabla F(\bw_t)$ than it would be using the standard momentum update. We augment this procedure with gradient clipping in Algorithm \ref{alg:nsgdclipigt} below, and provide its analysis in Theorems \ref{thm:nsgdclipigt} and \ref{thm:nsgdclipburninigt}, which are directly analogous to Theorems \ref{thm:nsgdclip} and \ref{thm:nsgdclipburnin}.
\begin{algorithm}
   \caption{NIGT with Clipping}
   \label{alg:nsgdclipigt}
   \begin{algorithmic}
      \STATE{\bfseries Input: } Initial Point $\bw_1$, learning rates $\eta$, momentum parameters $\alpha$, clipping parameter $\tau$, time horizon $T$:
      \STATE Set $\bm_1 = 0$.
      \FOR{$t=1\dots T$}
      \STATE Sample $z_t\sim P_z$.
      \STATE $\bx_t = \bw_t + \frac{\beta(\bw_t - \bw_{t-1})}{1-\beta}$
      \STATE Set $\bgclip_t = \frac{\nabla f(\bx_t, z_t)}{\|\nabla f(\bx_t, z_t)\|}\min(\tau, \|\nabla f(\bx_1,z_t)\|)$.
      \STATE 
      \STATE Set $\bm_t = \beta \bm_{t-1} +  (1-\beta) \bgclip_t$.
      \STATE Set $\bw_{t+1} = \bw_t  - \eta \frac{\bm_t}{\|\bm_t\|}$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}




\begin{restatable}{Theorem}{thmnsgdclipigt}\label{thm:nsgdclipigt}
Suppose $\E_z[\|\nabla f(\bw,z)-\nabla F(\bx)\|^\power]\le G^\power$ for all $\bx$ for some $G$. Suppose $F$ is $L$-smooth and $\rho$-second-order smooth. Set $\beta=1-\alpha$, $\alpha = \frac{b}{T^{\frac{2\power}{5\power-3}}}$ and $\eta = \frac{c}{T^{\frac{3\power -1}{5\power-3}}}$ for arbitrary constants $b$ and $c$ satisfying $\alpha \le 1$, and set $\tau=\frac{G}{\alpha^{1/\power}}$. Then with probability at least $1-\delta$:
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|&\le O\left(\frac{\log(T/\delta)}{ T^{\frac{2\power-2}{5\power-3}}}\right)
\end{align*}
where the big-Oh hides constant that depend on $L$, $\rho$, $G$, $b$, $c$, and $F(\bw_1)-F(\bw_{T+1})$, but not $T$ or $\delta$.
\end{restatable}

We also have a direct analog of Theorem \ref{thm:nsgdclipburnin}
\begin{restatable}{Theorem}{thmnsgdclipburninigt}\label{thm:nsgdclipburninigt}
Under the assumptions of Theorem \ref{thm:nsgdclipigt}, define the constants:
\begin{align*}
K&=6\max(1,\log(3T/\delta)) + 3\max(1,\log(3T/\delta)) + 1\\
    Z&= \frac{\rho c^2}{b^2} + GK b^{\frac{\power-1}{\power}}
\end{align*}
Then, with probability at least $1-\delta$, if
\begin{align*}
t\ge \mathcal{T}=\frac{T^\frac{\power}{3\power-2}}{b}\left(\frac{\power-1}{3\power-2}\log(T) +\log(G)- \log(Z)\right)
\end{align*}
Then we have
\begin{align*}
    \|\bm_t-\nabla F(\bx_t)\|&\le\frac{2Z}{T^{\frac{\power-1}{3\power-2}}}
\end{align*}
And so long as
\begin{align}
\|\bm_t\|\ge 2\left(\frac{22Z }{T^{\frac{3\power-1}{5\power-3}}} + \frac{3Lc}{2T^{\frac{3\power-1}{5\power-3}}}\right)\label{eqn:mconditionigt}
\end{align}
we have $F(\bw_{t+1})< F(\bw_t)-\frac{\eta}{6} \|\bm_t\|$. Moreover, if (\ref{eqn:mconditionigt}) is ever not satisfied, we must have 
\begin{align*}
    \|\nabla F(\bw_t)\|\le \frac{46 Z}{T^{\frac{3\power-1}{3\power-3}}} + \frac{6Lc}{2T^{\frac{3\power-1}{5\power-3}}}
\end{align*}
Finally, if $t$ is the iteration with smallest value of $\|\bm_t\|$ such that $t\ge \mathcal{T}$, we have with probability at least $1-\delta$:
\begin{align*}
    \|\nabla F(\bw_t)\|\le O\left(\frac{\log(T/\delta)}{T^{\frac{\power-1}{3\power-2}}}\right)
\end{align*}
\end{restatable}

\begin{proof}[Proof of Theorem \ref{thm:nsgdclipigt}]
The start of our proof is very similar to that of Theorem 3 in \cite{cutkosky2020momentum}.
As in the proof of Theorem \ref{thm:nsgdclip}, define $\hat\epsilon_t = \bm_t - \nabla F(\bw_t)$ and $\epsilon_t=\bgclip_t - \nabla F(\bw_t)$. Also (and as a departure from Theorem \ref{thm:nsgdclip}), define $S(a,b) = \nabla F(a)-\nabla F(b) - \nabla^2F(b)(a-b)$. Then we have a recursion:
\begin{align*}
    \bm_{t+1} &= (1-\alpha)(\nabla F(\bw_t) + \hat\epsilon_t) + \alpha \bgclip_t\\
    &=  (1-\alpha)(\nabla F(\bw_{t+1})+\nabla^2F(\bw_{t+1})(\bw_t-\bw_{t+1}) )\\
    &\quad+(1-\alpha)(S(\bw_t,\bw_{t+1})+ \hat\epsilon_t)\\
    &\quad+\alpha(\nabla F(\bw_{t+1}) + \nabla^2F(\bw_{t+1})(\bw_{t+1}-\bx_{t+1}))\\
    &\quad+\alpha(S(\bx_{t+1},\bw_{t+1}) +\epsilon_{t+1}))
    \intertext{Now, observe that by definition of $\bx_{t+1}$, the hessian-dependent terms cancel:}
    &=\nabla F(\bw_{t+1}) + (1-\alpha)(S(\bw_t,\bw_{t+1}) + \hat\epsilon_t)\\
    &\quad+\alpha( S(\bx_{t+1},\bw_{t+1}) + \epsilon_{t+1})\\
    \hat \epsilon_{t+1} &= (1-\alpha)(S(\bw_t,\bw_{t+1}) + \hat\epsilon_t)\\
    &\quad+\alpha( S(\bx_{t+1},\bw_{t+1}) + \epsilon_{t+1})\\
    \hat \epsilon_{t+1} &= (1-\alpha)^t\hat \epsilon_1 + \alpha \sum_{t'=1}^t (1-\alpha)^{t'} \epsilon_{t+1-t'}\\
    &\quad+(1-\alpha)\sum_{t'=1}^t(1-\alpha)^{t'}S(\bw_{t-t'},\bw_{t-t'+1})\\
    &\quad+\alpha\sum_{t'=1}^t(1-\alpha)^{t'}S(\bx_{t-t'+1},\bw_{t-t'+1})\\
    \|\hat\epsilon_{t+1}\|&\le (1-\alpha)^t\hat \|\epsilon_1\| + \alpha \left\|\sum_{t'=1}^t (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|\\
    &\quad+(1-\alpha)\left\|\sum_{t'=1}^t(1-\alpha)^{t'}S(\bw_{t-t'},\bw_{t-t'+1})\right\|\\
    &\quad+\alpha\left\|\sum_{t'=1}^t(1-\alpha)^{t'}S(\bx_{t-t'+1},\bw_{t-t'+1})\right\|
    \intertext{Now, by second-order smoothness, we have $\|S(a,b)\|\le \frac{\rho}{2}\|a-b\|^2$, so that:}
    &\le  (1-\alpha)^t\hat \|\epsilon_1\| + \alpha \left\|\sum_{t'=1}^t (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|\\
    &\quad+\frac{(1-\alpha)\rho\eta^2}{\alpha }\sum_{t'=1}^t(1-\alpha)^{t'}\\
    &\le  (1-\alpha)^t\hat \|\epsilon_1\| + \alpha \left\|\sum_{t'=1}^t (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|\\
    &\quad+\frac{(1-\alpha)\rho\eta^2}{\alpha^2 }
\end{align*}
Now, by exactly the same argument as in Theorem \ref{thm:nsgdclip}, defining $D_\delta=\max(1,\log(1/\delta))$ we have with probability at least $1-\delta/T$:
\begin{align}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t G + \frac{(1-\alpha)\rho\eta^2}{\alpha^2 }+ 6\alpha\tau D_\delta\nonumber\\
    &\quad+ 3\sqrt{ \alpha G^\power\tau^{2-\power}D_\delta}+\frac{G^\power}{ \tau^{\power-1}}\nonumber
    \intertext{
Then, with $\tau=\frac{G}{\alpha^{1/\power}}$, this becomes:}
&\le (1-\alpha)^t G + \frac{(1-\alpha)\rho\eta^2}{\alpha^2}\nonumber\\
&\mkern-50mu+G\alpha^{1-1/\power}\left[6D_\delta + 3\sqrt{D_\delta} + 1\right]\nonumber\\
    % &\quad\left.+\frac{2}{3} + \sqrt{2^{\power-1}} + 2^{\power-1}\right]\\
    &=(1-\alpha)^tG+ \frac{(1-\alpha)\rho\eta^2}{\alpha^2} + G\alpha^{1-1/\power}K\label{eqn:hatepsboundigt}
\end{align}
where we again define the constant $K=6D_\delta + 3\sqrt{D_\delta} + 1$.


Now, we have from \cite{cutkosky2020momentum} Lemma 2:
\begin{align*}
    \sum_{t=1}^T \|\nabla F(\bw_t)\|&\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}\\
    &\quad+8\sum_{t=1}^T \|\hat\epsilon_t\|
    \intertext{so with probability at least $1-\delta$:}
    &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}\\
    &\quad+8\sum_{t=1}^T(1-\alpha)^tG+ \frac{(1-\alpha)\rho\eta^2}{\alpha^2}\\
    &\quad+ G\alpha^{1-1/\power}K\\
    &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}\\
    &\quad+\frac{8G(1-\alpha)}{\alpha} +\frac{(1-\alpha)T\rho\eta^2}{\alpha^2} \\
    &\quad+ GT\alpha^{1-1/\power}K
\end{align*}
Now set $\alpha = \frac{b}{T^{\frac{2\power}{5\power-3}}}$ and $\eta = \frac{c}{T^{\frac{3\power -1}{5\power-3}}}$. This yields with probability at least $1-\delta$:
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|&\le O\left( T^{\frac{2-2\power}{5\power-3}}\log(T/\delta)\right)
\end{align*}


\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:nsgdclipburninigt}]
Use the settings $\eta=\frac{c}{T^{\frac{3\power-1}{5\power-3}}}$ and $\alpha = \frac{b}{T^{\frac{2\power}{5\power-3}}}$ and notice that from equation (\ref{eqn:hatepsboundigt}) that with probability $1-\delta$, for all $t$:
\begin{align*}
    \|\hat \epsilon_{t+1}\|
    &\le (1-\alpha)^tG+ \frac{(1-\alpha)\rho\eta^2}{\alpha^2} + G\alpha^{1-1/\power}K\\
    &=(1-\alpha)^t G + \frac{\rho c^2}{b^2T^{\frac{2\power-2}{5\power-3}}} + \frac{GK b^{\frac{\power-1}{\power}}}{T^{\frac{2\power-2}{5\power-3}}}\\
    &=(1-\alpha)^t G + \frac{Z}{T^{\frac{2\power-2}{5\power-3}}}
\end{align*}

Again, we have the identity:
\begin{align*}
    \log(1-\alpha)&\le -\alpha\\
    \log\left(G(1-\alpha)^t)\right) &\le -t\alpha +\log(G)
\end{align*}
Therefore, if $t$ satisfies:
\begin{align*}
    t\ge \frac{T^\frac{2\power}{5\power-3}}{b}\left(\frac{2\power-2}{5\power-3}\log(T) +\log(G) - \log\left(Z\right)\right)
\end{align*}
we have with probability at least $1-\delta$:
\begin{align*}
\|\hat \epsilon_{t+1}\|&\le \frac{2Z}{T^{\frac{2\power-2}{5\power-3}}}
\end{align*}
Next, again from Lemma 2 of \cite{cutkosky2020momentum},
\begin{align*}
    F(\bw_{t+1})&\le F(\bw_t) - \frac{\eta}{3}\|\nabla F(\bw_t)\| + \frac{8\eta}{3}\|\hat\epsilon_t\| + \frac{L\eta^2}{2}\\
    &\le F(\bw_t) - \frac{\eta}{3}\|\bm_t\| + \frac{11\eta}{3}\|\hat\epsilon_t\| + \frac{L\eta^2}{2}\\
    &\le F(\bw_t) - \frac{\eta}{3}\|\bm_t\| +\frac{\eta}{3}\left(\frac{22Z }{T^{\frac{3\power-1}{5\power-3}}} + \frac{3Lc}{2T^{\frac{3\power-1}{5\power-3}}}\right)
\end{align*}

Now, analogously to Theorem \ref{thm:nsgdclipburnin}, we argue that if $\|\bm_t\|\ge 2\left(\frac{22Z }{T^{\frac{3\power-1}{5\power-3}}} + \frac{3Lc}{2T^{\frac{3\power-1}{5\power-3}}}\right)$, then $F(\bw_{t+1})\le F(\bw-t) - \frac{\eta}{6}\|\bm_t\|$.

The last part of the Theorem follows from an identical case-work argument to that of Theorem \ref{thm:nsgdclipburnin}.
% For the last part of the Theorem, observe that since $F$ is $G$-Lipschitz, we must have that 
% \begin{align*}
%     F(\bw_{\mathcal{T}})-F(\bw_1)\le G\mathcal{T} \eta=O(\log(T))
% \end{align*}
% so that $F(\bw_{\mathcal{T}}) - F(\bw_{T+1}) \le O(F(\bw_1)-F(\bw_{T+1}) + \log(T))$. Now consider two cases, either 
% \begin{align*}
%     \min_{t\ge \mathcal{T}} \|\bm_t\|\le 2\left(\frac{22Z }{T^{\frac{3\power-1}{5\power-3}}} + \frac{3Lc}{2T^{\frac{3\power-1}{5\power-3}}}\right)
% \end{align*}
% or not. In the first case, by our bound on $\|\hat \epsilon_t\|$, the desired bound on $\|\nabla F(\bw_t)\|$ follows. In the latter case, we have
% \begin{align*}
%      F(\bw_{T+1})&\le F(\bw_{\mathcal{T}})-\frac{\eta}{6}\sum_{t=\mathcal{T}}^T \|\bm_t\|
% \end{align*}
% So that 
% \begin{align*}
%     &\min_{t\ge \mathcal{T}} \|\bm_t\| \le O\left(\frac{F(\bw_1)-F(\bw_{T+1}) + \log(T)}{T\eta}\right) \\
%     &= \tilde O\left(\frac{1}{T^{\frac{3\power-1}{5\power-3}}}\right)
% \end{align*}
% And so again the result follows from our bound on $\|\hat\epsilon_t\|$. 
\end{proof}

Finally, we note that we have a statement about the last iterate of Algorithm \ref{alg:nsgdclipigt} that is directly analogous to Corollary \ref{thm:lastiterate} (the proof is essentially identical):
\begin{Corollary}\label{thm:lastiterateigt}
Under the notation and assumptions of Theorem \ref{thm:nsgdclipburninigt}, with probability at least $1-\delta$, there exists some $\hat w$ such that both of the following inequalities hold:
\begin{align*}
    \|\nabla F(\hat w)\|&\le O\left(\frac{\log(T/\delta)}{T^{\frac{3\power-1}{5\power-2}}}\right)\\
    F(\bw_T) &\le F(\hat w)
\end{align*}
where $\bw_T$ is the last iterate of Algorithm \ref{alg:nsgdclipigt}
\end{Corollary}


==> sgd_arxiv.tex <==
\section{Normalized SGD with Momentum}\label{sec:normalized}
In this section, we describe our algorithms for finding critical points with high probability in non-convex objectives. Our analysis makes use of gradient clipping, momentum, and normalized updates. Clipping is a standard technique for mitigating the effect of heavy tails, essentially by throwing out outlier data. Momentum is useful as it intuitively averages together many clipped gradients, resulting in a gradient estimate that concentrates about its mean with high probability. Normalizing the updates allows for significantly simplified analyses because the bias terms introduced by the moving average in momentum are now very precisely controlled by the learning rate, as originally analyzed in \citep{cutkosky2020momentum}.
\begin{algorithm}
   \caption{Normalized SGD with Clipping and Momentum}
   \label{alg:nsgdclip}
   \begin{algorithmic}
      \STATE{\bfseries Input: } Initial Point $\bw_1$, learning rates $\eta$, momentum parameters $\alpha$, clipping parameter $\tau$, time horizon $T$:
      \STATE Set $\bm_1 = 0$.
      \FOR{$t=1\dots T$}
      \STATE Sample $z_t\sim P_z$.
      \STATE Set $\bgclip_t = \frac{\nabla f(\bw_t, z_t)}{\|\nabla f(\bw_t, z_t)\|}\min(\tau, \|\nabla f(\bw_1,z_t)\|)$.
      \STATE Set $\bm_t = \beta \bm_{t-1}+ (1-\beta) \bgclip_t$.
      \STATE Set $\bw_{t+1} = \bx_t  - \eta \frac{\bm_t}{\|\bm_t\|}$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}



\begin{restatable}{Theorem}{thmnsgdclip}\label{thm:nsgdclip}
Suppose $\E_z[\|\nabla f(\bw,z)-\nabla F(\bx)\|^\power]\le G^\power$ for all $\bx$ for some $G$. Suppose $F$ is $L$-smooth. Set $\beta=1-\alpha$, $\alpha = \frac{b}{T^{\frac{\power}{3\power-2}}}$ and $\eta = \frac{c}{T^{\frac{2\power -1}{3\power-2}}}$ for arbitrary constant $b$ and $c$ satisfying $\alpha \le 1$ and set $\tau=G/\alpha^{1/\power}$. Then with probability at least $1-\delta$:
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|&\le  O\left(\frac{\log(T/\delta)}{T^{\frac{\power-1}{3\power-2}}}\right)
\end{align*}
where the big-Oh hides constant that depend on $L$, $G$ $b$, $c$, and $F(\bw_1)-F(\bw_{T+1})$, but not $T$ or $\delta$.
\end{restatable}
This Theorem provides an analog of the standard in-expectation result for non-convex optimization, but now the result holds with high-probability. Note that this matches the in-expectation convergence rates from \citet{zhang2020adaptive}. The next Theorem takes this theme one step further: it shows that after a brief ``burn-in'' period, the decrease in objective value will in fact be \emph{monotonic} with high probability:
\begin{restatable}{Theorem}{thmnsgdclipburnin}\label{thm:nsgdclipburnin}
Under the assumptions of Theorem \ref{thm:nsgdclip}, define the constants:
\begin{align*}
K&=6\max(1,\log(3T/\delta)) + 3\max(1,\log(3T/\delta)) + 1\\
    Z&= \frac{cL}{b}+GKb^{\frac{\power-1}{\power}}
\end{align*}
Then, with probability at least $1-\delta$, if
\begin{align*}
t\ge \mathcal{T}=\frac{T^\frac{\power}{3\power-2}}{b}\left(\frac{\power-1}{3\power-2}\log(T) +\log(G)- \log(Z)\right)
\end{align*}
Then we have
\begin{align*}
    \|\bm_t-\nabla F(\bw_t)\|&\le\frac{2Z}{T^{\frac{\power-1}{3\power-2}}}
\end{align*}
And so long as
\begin{align}
\|\bm_t\|\ge 2\left(\frac{22 Z}{T^{\frac{\power-1}{3\power-2}}} + \frac{3Lc}{2T^{\frac{2\power-1}{3\power-2}}}\right)\label{eqn:mcondition}
\end{align}
we have $F(\bw_{t+1})< F(\bw_t)-\frac{\eta}{2}\|\bm_t\|$. Moreover, if (\ref{eqn:mcondition}) is ever not satisfied, we must have 
\begin{align*}
    \|\nabla F(\bw_t)\|\le \frac{46 Z}{T^{\frac{\power-1}{3\power-2}}} + \frac{6Lc}{2T^{\frac{2\power-1}{3\power-2}}}
\end{align*}
Finally, if $t$ is the iteration with smallest value of $\|\bm_t\|$ such that $t\ge \mathcal{T}$, we have with probability at least $1-\delta$:
\begin{align*}
\|\nabla F(\bw_t)\| \le O\left(\frac{\log(T/\delta)}{T^{\frac{\power-1}{3\power-2}}}\right)
\end{align*}
\end{restatable}

Theorem \ref{thm:nsgdclipburnin} shows that after a small burn-in period $\mathcal{T}=o(T)$, $\bm_t$ is very likely to be an extremely good estimate of the true gradient $\nabla F(\bx_t)$. Moreover, we can empirically detect this event by monitoring the norm of the exponentially weighted moving average $\bm$. This burn-in period is especially interesting given the success of learning rate schedules that incorporate a ``warm-up'' component, in which the learning rate actually increases during the first iterations. Our result seems to hint at a mechanism for this schedule: by keeping the learning rate small during the burn-in period, we can limit any increase in the objective value until we reach the stage at which it begins to decrease steadily.

Further, Theorem \ref{thm:nsgdclipburnin} provides a very concrete algorithm to find critical points: after the burn-in period of $\tilde O(T^{\frac{\power}{3\power-2}})$ iterates, we can simply return the point $\bx_t$ with the smallest value of $\|\bm_t\|$. Intuitively, this works because the objective value can only increase by a total of $O(T^{\frac{\power}{3\power-2}}\eta)=O(T^{\frac{1-\power}{3\power-2}})=O(1)$ during the burn-in period so even without a learning rate ``warm-up'', we should not expect the burn-in period to have too significant an effect on the objective value. After the burnin-in period, $\bm_t$ is always very close to $\nabla F(\bw_t)$, so we make steady progress until a critical point is encountered.

\begin{proof}[Proof of Theorem \ref{thm:nsgdclip}]
Define $\hat \epsilon_t = \bm_t - \nabla F(\bw_t)$. and $\epsilon_t = \bgclip_t - \nabla F(\bw_t)$. Also, define $S(a,b)=\nabla F(a)-\nabla F(b)$. By smoothness, we have $\|S(\bw_t,\bw_{t+1})\|\le L\|\bw_t-\bw_{t+1}\|$

If we define $\bw_0=\bw_1$, then we have the following recursive formulation for any $t\ge 0$:
\begin{align*}
    \bm_{t+1} &= (1-\alpha) (\nabla F(\bw_t) + \hat \epsilon_t) + \alpha\bg^{\text{ clip}}_{t+1}\\
    &=\nabla F(\bw_{t+1}) + (1-\alpha)(S(\bw_t,\bw_{t+1})+\hat \epsilon_t) + \alpha\epsilon_{t+1}\\
    \hat \epsilon_{t+1}&= (1-\alpha)S(\bw_t,\bw_{t+1})+(1-\alpha)\hat \epsilon_t + \alpha \epsilon_{t+1}
\end{align*}
Now, we unravel the recursion for $t+1$ iterations:
\begin{align*}
    \hat \epsilon_{t+1}&=(1-\alpha)^t\hat \epsilon_0 +\alpha\sum_{t'=0}^{t} (1-\alpha)^{t'} \epsilon_{t+1-t'}+ (1-\alpha)\sum_{t'=0}^{t}(1-\alpha)^{t'} S(\bw_{t-t'},\bw_{t+1-t'})
\end{align*}
Next, take the magnitude of both sides and use triangle inequality (using the fact that $\|S(\bw_a,\bw_{t+1})\|\le L\eta$):
\begin{align*}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t\|\hat\epsilon_0\| +\alpha\left\|\sum_{t'=0}^{t} (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|+ (1-\alpha)\eta L \sum_{t'=0}^{t}(1-\alpha)^{t'}\\
    &\le (1-\alpha)^t G + \frac{(1-\alpha)\eta L}{\alpha}+\alpha\left\|\sum_{t'=0}^{t} (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|
\end{align*}
where in the second line we have used $\bm_0=0$ and $\|\nabla F(\bw_0)\|\le G$, which follows since $\|\nabla F(\bw_0)\|\le \E_z[\|\nabla f(\bw_0,z)\|^\power]^{1/\power}=G$.

Now, by Lemma \ref{thm:thresholdsimple}, with probability at least $1-\delta/T$:
\begin{align*}
    \left\|\sum_{t'=0}^{t} (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|&\le  6\tau\max(1,\log(3T/\delta))+\sum_{t'=0}^t \frac{(1-\alpha)^{t'}G^\power}{\tau^{\power-1}}\\
    &\quad\quad+3\sqrt{\sum_{t'=0}^t(1-\alpha)^{2t'}G^\power \tau^{2-\power}\max(1,\log(3T/\delta))}\\
    &\le 6\tau\max(1,\log(3T/\delta))+\frac{G^\power}{\alpha \tau^{\power-1}} +\frac{3\sqrt{G^\power \tau^{2-\power}\max(1,\log(3T/\delta))}}{\sqrt{\alpha}}
\end{align*}

Therefore, with probability at least $1-\delta/T$:
\begin{align}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t G + \frac{(1-\alpha)\eta L}{\alpha} + 6\alpha\tau\max(1,\log(3T/\delta))\nonumber\\
    &\quad+ 3\sqrt{ \alpha G^\power\tau^{2-\power}\max(1,\log(3T/\delta))}+\frac{G^\power}{ \tau^{\power-1}}\nonumber\\
    % &\quad+\frac{4\tau \alpha}{3}\log\left[\frac{50}{\delta}\left(\frac{T}{\tau}+1\right)\right]+\sqrt{2\alpha\log\left[\frac{50}{\delta}\left(\frac{T}{\tau}+1\right)\right]G^\power \tau^{2-\power}}\\
    % &\quad+\frac{2\tau \alpha}{3} + \sqrt{2^{\power-1}\alpha G^\power \tau^{2-\power}} + \frac{2^{\power-1}G^\power}{ \tau^{\power-1}}
    \intertext{
Now, with $\tau=\frac{G}{\alpha^{1/\power}}$, and $D_\delta=\max(1,\log(3T/\delta))$ this becomes:}
&\le (1-\alpha)^t G + \frac{(1-\alpha)\eta L}{\alpha} +G\alpha^{1-1/\power}\left[6D_\delta + 3\sqrt{D_\delta} + 1\right]\nonumber\\
    % \frac{4}{3}\log\left[\frac{50}{\delta}\left(\frac{T\alpha^{1/\power}}{G}+1\right)\right]+\sqrt{2\log\left[\frac{50}{\delta}\left(\frac{T\alpha^{1/\power}}{G}+1\right)\right]}\right.\\
    % &\quad\left.+\frac{2}{3} + \sqrt{2^{\power-1}} + 2^{\power-1}\right]\\
    &=(1-\alpha)^tG+ \frac{(1-\alpha)\eta L}{\alpha} + G\alpha^{1-1/\power}K\label{eqn:hatepsbound}
\end{align}
where we define the constant $K=6D_\delta + 3\sqrt{D_\delta} + 1$. 


Now, we have from \citet{cutkosky2020momentum} Lemma 2:
\begin{align*}
   \sum_{t=1}^T \|\nabla F(\bw_t)\|&\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+8\sum_{t=1}^T \|\hat\epsilon_t\|
    \intertext{so with probability at least $1-\delta$:}
    &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+8\sum_{t=1}^T(1-\alpha)^tG+ \frac{(1-\alpha)\eta L}{\alpha} + G\alpha^{1-1/\power}K\\
    &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+\frac{8G(1-\alpha)}{\alpha}+ \frac{(1-\alpha)\eta T L}{\alpha} + GT\alpha^{1-1/\power}K
\end{align*}
Now set $\alpha = \frac{b}{T^{\frac{\power}{3\power-2}}}$ and $\eta = \frac{c}{T^{\frac{2\power -1}{3\power-2}}}$. This yields:
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|&\le  O\left( T^{\frac{1-\power}{3\power-2}}\log(T/\delta)\right)
\end{align*}
\end{proof}

The proof of Theorem \ref{thm:nsgdclipburnin} follows essentially the same idea as that of Theorem \ref{thm:nsgdclip}. However, this time we use the explicit bound on $\|\hat\epsilon_t\|$ and observe that after the burn-in period, the contribution from $\|\epsilon_1\|$ has decreased exponentially to be insignificant, and so $\bm_t$ will be a very high-quality estimate of $\nabla F(\bx_t)$ at every single iteration.

\begin{proof}[Proof of Theorem \ref{thm:nsgdclipburnin}]
Use the settings $\eta=\frac{c}{T^{\frac{2\power-1}{3\power-2}}}$ and $\alpha = \frac{b}{T^{\frac{\power}{3\power-2}}}$ and notice that from equation (\ref{eqn:hatepsbound}) that with probability $1-\delta$, for all $t$:
\begin{align*}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t G + \frac{cL}{bT^{\frac{\power-1}{3\power-2}}}+\frac{GKb^{\frac{\power-1}{\power}}}{T^{\frac{\power-1}{3\power-2}}}\\
    &=(1-\alpha)^t G + \frac{Z}{T^{\frac{\power-1}{3\power-2}}}
\end{align*}
Further, we have
\begin{align*}
    \log(1-\alpha)&\le -\alpha\\
    \log\left(G(1-\alpha)^t)\right) &\le -t\alpha +\log(G)
\end{align*}
Therefore, if $t$ satisfies:
\begin{align*}
    t\ge \frac{T^\frac{\power}{3\power-2}}{b}\left(\frac{\power-1}{3\power-2}\log(T) +\log(G) - \log\left(Z\right)\right)
\end{align*}
we have with probability at least $1-\delta$:
\begin{align*}
\|\hat \epsilon_{t+1}\|&\le \frac{2Z}{T^{\frac{\power-1}{3\power-2}}}
\end{align*}
This implies the bound on $\|\nabla F(\bw_t)\|$ when $\|\bm_t\|$ is smaller than the threshold described in the Theorem statement. Next, again from Lemma 2 of \citet{cutkosky2020momentum},
\begin{align*}
    F(\bw_{t+1})&\le F(\bw_t) - \frac{\eta}{3}\|\nabla F(\bw_t)\| + \frac{8\eta}{3}\|\hat\epsilon_t\| + \frac{L\eta^2}{2}\\
    &\le F(\bw_t) - \frac{\eta}{3}\|\bm_t\| + \frac{11\eta}{3}\|\hat\epsilon_t\| + \frac{L\eta^2}{2}\\
    &\le F(\bw_t) - \frac{\eta}{3}\|\bm_t\| +\frac{\eta}{3}\left(\frac{22Z }{T^{\frac{\power-1}{3\power-2}}} + \frac{3Lc}{2T^{\frac{2\power-1}{3\power-2}}}\right)
\end{align*}
from which we can conclude that if $\|\bm_t\|\ge 2\left(\frac{22Z }{T^{\frac{\power-1}{3\power-2}}} + \frac{3Lc}{2T^{\frac{2\power-1}{3\power-2}}}\right)$, $F(\bw_{t+1})\le F(\bw-t) - \frac{\eta}{6}\|\bm_t\|$.

Now, for the final part of the Theorem, observe that since $F$ is $G$-Lipschitz, we must have that 
\begin{align*}
    F(\bw_{\mathcal{T}})-F(\bw_1)\le G\mathcal{T} \eta=O(\log(T))
\end{align*}
so that $F(\bw_{\mathcal{T}}) - F(\bw_{T+1}) \le O(F(\bw_1)-F(\bw_{T+1}) + \log(T))$. Now consider two cases, either 
\begin{align*}
    \min_{t\ge \mathcal{T}} \|\bm_t\|\le 2\left(\frac{22Z }{T^{\frac{\power-1}{3\power-2}}} + \frac{3Lc}{2T^{\frac{2\power-1}{3\power-2}}}\right)
\end{align*}
or not. In the first case, by our bound on $\|\hat \epsilon_t\|$, the desired bound on $\|\nabla F(\bw_t)\|$ follows. In the latter case, we have
\begin{align*}
     F(\bw_{T+1})&\le F(\bw_{\mathcal{T}})-\frac{\eta}{6}\sum_{t=\mathcal{T}}^T \|\bm_t\|
\end{align*}
So that 
\begin{align*}
    \min_{t\ge \mathcal{T}} \|\bm_t\| \le O\left(\frac{F(\bw_1)-F(\bw_{T+1}) + \log(T)}{T\eta}\right) = \tilde O\left(\frac{1}{T^{\frac{2\power-1}{3\power-2}}}\right)
\end{align*}
And so again the result follows from our bound on $\|\hat\epsilon_t\|$. 
\end{proof}

In addition to providing a method for identifying critical points, Theorem \ref{thm:nsgdclipburnin} also provides an intuitively desirable guarantee about the \emph{last-iterate} of the algorithm $\bw_T$. Specifically, one can easily check that the following Corollary:
\begin{Corollary}\label{thm:lastiterate}
Under the notation and assumptions of Theorem \ref{thm:nsgdclipburnin}, with probability at least $1-\delta$, there exists some $\hat w$ such that both of the following inequalities hold:
\begin{align*}
    \|\nabla F(\hat w)\|&\le O\left(\frac{\log(T/\delta)}{T^{\frac{\power-1}{3\power-2}}}\right)\\
    F(\bw_T) &\le F(\hat w)
\end{align*}
where $\bw_T$ is the last iterate of Algorithm \ref{alg:nsgdclip}
\end{Corollary}
\begin{proof}
Set $\hat w$ to be the last iterate for which condition \ref{eqn:mcondition} does not hold. Then the result is immediately implied by Theorem \ref{thm:nsgdclip}.
\end{proof}

In most applications we are not actually interested in finding critical points, but instead wish to actually minimize the objective $F$. This observation tells us that our objective value is at least never worse than it would have been if had indeed searched specifically for a critical point. Moreover, by providing a guarantee about $\bw_T$, we have a closer match to practical use-cases: many of the theoretical analyses of non-convex stochastic gradient methods \citep{ghadimi2013stochastic, ward2019adagrad,li2019convergence} only show that a \emph{randomly selected iterate} has a small gradient norm. In contrast, Corollary \ref{thm:lastiterate} provides a non-asymptotic guarantee for the final iterate, which is the iterate most likely to be deployed after training in practice.

\section{Second-Order Smooth Losses}\label{sec:igt}
In this section, we provide our extension to losses that are \emph{second order smooth}. The overall method is very similar: we employ normalized SGD with momentum. However, in order to take advantage of the second-order smoothness, we will need to use a more advanced form of momentum. Specifically, we use implicit gradient transport \citep{arnold2019reducing}, as implemented by \citet{cutkosky2020momentum} in the NIGT algorithm. This algorithm replaces the standard momentum update with an extrapolation procedure:
\begin{align*}
    \bm_t = \beta \bm_{t-1} +  (1-\beta) \nabla f\left(\bw_t + \frac{\beta(\bw_t - \bw_{t-1})}{1-\beta}, z_t\right)
\end{align*}
By evaluating the gradient at the ``shifted'' point $\bw_t + \frac{\beta(\bw_t - \bw_{t-1})}{1-\beta}$ and performing a second-order Taylor expansion enabled by the second-order smoothness assumption, it is possible to show that $\bm_t$ is a less-biased estimate of $\nabla F(\bw_t)$ than it would be using the standard momentum update. We augment this procedure with gradient clipping in Algorithm \ref{alg:nsgdclipigt} below, and provide its analysis in Theorems \ref{thm:nsgdclipigt} and \ref{thm:nsgdclipburninigt}, which are directly analogous to Theorems \ref{thm:nsgdclip} and \ref{thm:nsgdclipburnin}.
\begin{algorithm}
   \caption{NIGT with Clipping}
   \label{alg:nsgdclipigt}
   \begin{algorithmic}
      \STATE{\bfseries Input: } Initial Point $\bw_1$, learning rates $\eta$, momentum parameters $\alpha$, clipping parameter $\tau$, time horizon $T$:
      \STATE Set $\bm_1 = 0$.
      \FOR{$t=1\dots T$}
      \STATE Sample $z_t\sim P_z$.
      \STATE $\bx_t = \bw_t + \frac{\beta(\bw_t - \bw_{t-1})}{1-\beta}$
      \STATE Set $\bgclip_t = \frac{\nabla f(\bx_t, z_t)}{\|\nabla f(\bx_t, z_t)\|}\min(\tau, \|\nabla f(\bx_1,z_t)\|)$.
      \STATE 
      \STATE Set $\bm_t = \beta \bm_{t-1} +  (1-\beta) \bgclip_t$.
      \STATE Set $\bw_{t+1} = \bw_t  - \eta \frac{\bm_t}{\|\bm_t\|}$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}




\begin{restatable}{Theorem}{thmnsgdclipigt}\label{thm:nsgdclipigt}
Suppose $\E_z[\|\nabla f(\bw,z)-\nabla F(\bx)\|^\power]\le G^\power$ for all $\bx$ for some $G$. Suppose $F$ is $L$-smooth and $\rho$-second-order smooth. Set $\beta=1-\alpha$, $\alpha = \frac{b}{T^{\frac{2\power}{5\power-3}}}$ and $\eta = \frac{c}{T^{\frac{3\power -1}{5\power-3}}}$ for arbitrary constants $b$ and $c$ satisfying $\alpha \le 1$, and set $\tau=\frac{G}{\alpha^{1/\power}}$. Then with probability at least $1-\delta$:
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|&\le O\left(\frac{\log(T/\delta)}{ T^{\frac{2\power-2}{5\power-3}}}\right)
\end{align*}
where the big-Oh hides constant that depend on $L$, $\rho$, $G$, $b$, $c$, and $F(\bw_1)-F(\bw_{T+1})$, but not $T$ or $\delta$.
\end{restatable}

We also have a direct analog of Theorem \ref{thm:nsgdclipburnin}
\begin{restatable}{Theorem}{thmnsgdclipburninigt}\label{thm:nsgdclipburninigt}
Under the assumptions of Theorem \ref{thm:nsgdclipigt}, define the constants:
\begin{align*}
K&=6\max(1,\log(3T/\delta)) + 3\max(1,\log(3T/\delta)) + 1\\
    Z&= \frac{\rho c^2}{b^2} + GK b^{\frac{\power-1}{\power}}
\end{align*}
Then, with probability at least $1-\delta$, if
\begin{align*}
t\ge \mathcal{T}=\frac{T^\frac{\power}{3\power-2}}{b}\left(\frac{\power-1}{3\power-2}\log(T) +\log(G)- \log(Z)\right)
\end{align*}
Then we have
\begin{align*}
    \|\bm_t-\nabla F(\bx_t)\|&\le\frac{2Z}{T^{\frac{\power-1}{3\power-2}}}
\end{align*}
And so long as
\begin{align}
\|\bm_t\|\ge 2\left(\frac{22Z }{T^{\frac{3\power-1}{5\power-3}}} + \frac{3Lc}{2T^{\frac{3\power-1}{5\power-3}}}\right)\label{eqn:mconditionigt}
\end{align}
we have $F(\bw_{t+1})< F(\bw_t)-\frac{\eta}{6} \|\bm_t\|$. Moreover, if (\ref{eqn:mconditionigt}) is ever not satisfied, we must have 
\begin{align*}
    \|\nabla F(\bw_t)\|\le \frac{46 Z}{T^{\frac{3\power-1}{3\power-3}}} + \frac{6Lc}{2T^{\frac{3\power-1}{5\power-3}}}
\end{align*}
Finally, if $t$ is the iteration with smallest value of $\|\bm_t\|$ such that $t\ge \mathcal{T}$, we have with probability at least $1-\delta$:
\begin{align*}
    \|\nabla F(\bw_t)\|\le O\left(\frac{\log(T/\delta)}{T^{\frac{\power-1}{3\power-2}}}\right)
\end{align*}
\end{restatable}

\begin{proof}[Proof of Theorem \ref{thm:nsgdclipigt}]
The start of our proof is very similar to that of Theorem 3 in \citep{cutkosky2020momentum}.
As in the proof of Theorem \ref{thm:nsgdclip}, define $\hat\epsilon_t = \bm_t - \nabla F(\bw_t)$ and $\epsilon_t=\bgclip_t - \nabla F(\bw_t)$. Also (and as a departure from Theorem \ref{thm:nsgdclip}), define $S(a,b) = \nabla F(a)-\nabla F(b) - \nabla^2F(b)(a-b)$. Then we have a recursion:
\begin{align*}
    \bm_{t+1} &= (1-\alpha)(\nabla F(\bw_t) + \hat\epsilon_t) + \alpha \bgclip_t\\
    &=  (1-\alpha)(\nabla F(\bw_{t+1})+\nabla^2F(\bw_{t+1})(\bw_t-\bw_{t+1}) )+(1-\alpha)(S(\bw_t,\bw_{t+1})+ \hat\epsilon_t)\\
    &\quad+\alpha(\nabla F(\bw_{t+1}) + \nabla^2F(\bw_{t+1})(\bw_{t+1}-\bx_{t+1}))+\alpha(S(\bx_{t+1},\bw_{t+1}) +\epsilon_{t+1}))
    \intertext{Now, observe that by definition of $\bx_{t+1}$, the hessian-dependent terms cancel:}
    &=\nabla F(\bw_{t+1}) + (1-\alpha)(S(\bw_t,\bw_{t+1}) + \hat\epsilon_t)+\alpha( S(\bx_{t+1},\bw_{t+1}) + \epsilon_{t+1})\\
    \hat \epsilon_{t+1} &= (1-\alpha)(S(\bw_t,\bw_{t+1}) + \hat\epsilon_t)+\alpha( S(\bx_{t+1},\bw_{t+1}) + \epsilon_{t+1})\\
    \hat \epsilon_{t+1} &= (1-\alpha)^t\hat \epsilon_1 + \alpha \sum_{t'=1}^t (1-\alpha)^{t'} \epsilon_{t+1-t'}+(1-\alpha)\sum_{t'=1}^t(1-\alpha)^{t'}S(\bw_{t-t'},\bw_{t-t'+1})\\
    &\quad+\alpha\sum_{t'=1}^t(1-\alpha)^{t'}S(\bx_{t-t'+1},\bw_{t-t'+1})\\
    \|\hat\epsilon_{t+1}\|&\le (1-\alpha)^t\hat \|\epsilon_1\| + \alpha \left\|\sum_{t'=1}^t (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|+(1-\alpha)\left\|\sum_{t'=1}^t(1-\alpha)^{t'}S(\bw_{t-t'},\bw_{t-t'+1})\right\|\\
    &\quad+\alpha\left\|\sum_{t'=1}^t(1-\alpha)^{t'}S(\bx_{t-t'+1},\bw_{t-t'+1})\right\|
    \intertext{Now, by second-order smoothness, we have $\|S(a,b)\|\le \frac{\rho}{2}\|a-b\|^2$, so that:}
    &\le  (1-\alpha)^t\hat \|\epsilon_1\| + \alpha \left\|\sum_{t'=1}^t (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|+\frac{(1-\alpha)\rho\eta^2}{\alpha }\sum_{t'=1}^t(1-\alpha)^{t'}\\
    &\le  (1-\alpha)^t\hat \|\epsilon_1\| + \alpha \left\|\sum_{t'=1}^t (1-\alpha)^{t'} \epsilon_{t+1-t'}\right\|+\frac{(1-\alpha)\rho\eta^2}{\alpha^2 }
\end{align*}
Now, by exactly the same argument as in Theorem \ref{thm:nsgdclip}, defining $D_\delta=\max(1,\log(1/\delta))$ we have with probability at least $1-\delta/T$:
\begin{align}
    \|\hat \epsilon_{t+1}\|&\le (1-\alpha)^t G + \frac{(1-\alpha)\rho\eta^2}{\alpha^2 }+ 6\alpha\tau D_\delta+ 3\sqrt{ \alpha G^\power\tau^{2-\power}D_\delta}+\frac{G^\power}{ \tau^{\power-1}}\nonumber
    \intertext{
Then, with $\tau=\frac{G}{\alpha^{1/\power}}$, this becomes:}
&\le (1-\alpha)^t G + \frac{(1-\alpha)\rho\eta^2}{\alpha^2}+G\alpha^{1-1/\power}\left[6D_\delta + 3\sqrt{D_\delta} + 1\right]\nonumber\\
    % &\quad\left.+\frac{2}{3} + \sqrt{2^{\power-1}} + 2^{\power-1}\right]\\
    &=(1-\alpha)^tG+ \frac{(1-\alpha)\rho\eta^2}{\alpha^2} + G\alpha^{1-1/\power}K\label{eqn:hatepsboundigt}
\end{align}
where we again define the constant $K=6D_\delta + 3\sqrt{D_\delta} + 1$.


Now, we have from \citep{cutkosky2020momentum} Lemma 2:
\begin{align*}
    \sum_{t=1}^T \|\nabla F(\bw_t)\|&\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+8\sum_{t=1}^T \|\hat\epsilon_t\|
    \intertext{so with probability at least $1-\delta$:}
    &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+8\sum_{t=1}^T(1-\alpha)^tG+ \frac{(1-\alpha)\rho\eta^2}{\alpha^2}+ G\alpha^{1-1/\power}K\\
    &\le \frac{3(F(\bw_1)-F(\bw_T))}{\eta } + \frac{3LT\eta}{2}+\frac{8G(1-\alpha)}{\alpha} +\frac{(1-\alpha)T\rho\eta^2}{\alpha^2} + GT\alpha^{1-1/\power}K
\end{align*}
Now set $\alpha = \frac{b}{T^{\frac{2\power}{5\power-3}}}$ and $\eta = \frac{c}{T^{\frac{3\power -1}{5\power-3}}}$. This yields with probability at least $1-\delta$:
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T \|\nabla F(\bw_t)\|&\le O\left( T^{\frac{2-2\power}{5\power-3}}\log(T/\delta)\right)
\end{align*}


\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:nsgdclipburninigt}]
Use the settings $\eta=\frac{c}{T^{\frac{3\power-1}{5\power-3}}}$ and $\alpha = \frac{b}{T^{\frac{2\power}{5\power-3}}}$ and notice that from equation (\ref{eqn:hatepsboundigt}) that with probability $1-\delta$, for all $t$:
\begin{align*}
    \|\hat \epsilon_{t+1}\|
    &\le (1-\alpha)^tG+ \frac{(1-\alpha)\rho\eta^2}{\alpha^2} + G\alpha^{1-1/\power}K\\
    &=(1-\alpha)^t G + \frac{\rho c^2}{b^2T^{\frac{2\power-2}{5\power-3}}} + \frac{GK b^{\frac{\power-1}{\power}}}{T^{\frac{2\power-2}{5\power-3}}}\\
    &=(1-\alpha)^t G + \frac{Z}{T^{\frac{2\power-2}{5\power-3}}}
\end{align*}

Again, we have the identity:
\begin{align*}
    \log(1-\alpha)&\le -\alpha\\
    \log\left(G(1-\alpha)^t)\right) &\le -t\alpha +\log(G)
\end{align*}
Therefore, if $t$ satisfies:
\begin{align*}
    t\ge \frac{T^\frac{2\power}{5\power-3}}{b}\left(\frac{2\power-2}{5\power-3}\log(T) +\log(G) - \log\left(Z\right)\right)
\end{align*}
we have with probability at least $1-\delta$:
\begin{align*}
\|\hat \epsilon_{t+1}\|&\le \frac{2Z}{T^{\frac{2\power-2}{5\power-3}}}
\end{align*}
Next, again from Lemma 2 of \citep{cutkosky2020momentum},
\begin{align*}
    F(\bw_{t+1})&\le F(\bw_t) - \frac{\eta}{3}\|\nabla F(\bw_t)\| + \frac{8\eta}{3}\|\hat\epsilon_t\| + \frac{L\eta^2}{2}\\
    &\le F(\bw_t) - \frac{\eta}{3}\|\bm_t\| + \frac{11\eta}{3}\|\hat\epsilon_t\| + \frac{L\eta^2}{2}\\
    &\le F(\bw_t) - \frac{\eta}{3}\|\bm_t\| +\frac{\eta}{3}\left(\frac{22Z }{T^{\frac{3\power-1}{5\power-3}}} + \frac{3Lc}{2T^{\frac{3\power-1}{5\power-3}}}\right)
\end{align*}

Now, analogously to Theorem \ref{thm:nsgdclipburnin}, we argue that if $\|\bm_t\|\ge 2\left(\frac{22Z }{T^{\frac{3\power-1}{5\power-3}}} + \frac{3Lc}{2T^{\frac{3\power-1}{5\power-3}}}\right)$, then $F(\bw_{t+1})\le F(\bw-t) - \frac{\eta}{6}\|\bm_t\|$.

The last part of the Theorem follows from an identical case-work argument to that of Theorem \ref{thm:nsgdclipburnin}.
% For the last part of the Theorem, observe that since $F$ is $G$-Lipschitz, we must have that 
% \begin{align*}
%     F(\bw_{\mathcal{T}})-F(\bw_1)\le G\mathcal{T} \eta=O(\log(T))
% \end{align*}
% so that $F(\bw_{\mathcal{T}}) - F(\bw_{T+1}) \le O(F(\bw_1)-F(\bw_{T+1}) + \log(T))$. Now consider two cases, either 
% \begin{align*}
%     \min_{t\ge \mathcal{T}} \|\bm_t\|\le 2\left(\frac{22Z }{T^{\frac{3\power-1}{5\power-3}}} + \frac{3Lc}{2T^{\frac{3\power-1}{5\power-3}}}\right)
% \end{align*}
% or not. In the first case, by our bound on $\|\hat \epsilon_t\|$, the desired bound on $\|\nabla F(\bw_t)\|$ follows. In the latter case, we have
% \begin{align*}
%      F(\bw_{T+1})&\le F(\bw_{\mathcal{T}})-\frac{\eta}{6}\sum_{t=\mathcal{T}}^T \|\bm_t\|
% \end{align*}
% So that 
% \begin{align*}
%     &\min_{t\ge \mathcal{T}} \|\bm_t\| \le O\left(\frac{F(\bw_1)-F(\bw_{T+1}) + \log(T)}{T\eta}\right) \\
%     &= \tilde O\left(\frac{1}{T^{\frac{3\power-1}{5\power-3}}}\right)
% \end{align*}
% And so again the result follows from our bound on $\|\hat\epsilon_t\|$. 
\end{proof}

Finally, we note that we have a statement about the last iterate of Algorithm \ref{alg:nsgdclipigt} that is directly analogous to Corollary \ref{thm:lastiterate} (the proof is essentially identical):
\begin{Corollary}\label{thm:lastiterateigt}
Under the notation and assumptions of Theorem \ref{thm:nsgdclipburninigt}, with probability at least $1-\delta$, there exists some $\hat w$ such that both of the following inequalities hold:
\begin{align*}
    \|\nabla F(\hat w)\|&\le O\left(\frac{\log(T/\delta)}{T^{\frac{3\power-1}{5\power-2}}}\right)\\
    F(\bw_T) &\le F(\hat w)
\end{align*}
where $\bw_T$ is the last iterate of Algorithm \ref{alg:nsgdclipigt}
\end{Corollary}

